Microscopic Derivation of Ginzburg-Landau Theory and the BCS Critical Temperature Shift in General External Fields

We consider the Bardeen-Cooper-Schrieffer (BCS) free energy functional with weak and macroscopic external electric and magnetic fields and derive the Ginzburg-Landau functional. We also provide an asymptotic formula for the BCS critical temperature as a function of the external fields. This extends our previous results in arXiv:2105.05623 for the constant magnetic field to general magnetic fields with a nonzero magnetic flux through the unit cell.

==> 4_Proofs/4.2_Representation_Formula.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Proof of Proposition \ref{BCS functional_identity}}
\label{BCS functional_identity_proof_Section}

We recall the definitions of $\Delta(X, r) = -2\, V\alpha_*(r) \Psi(X)$ in \eqref{Delta_definition}, the Hamiltonian $H_\Delta$ in \eqref{HDelta_definition} and $\Gamma_\Delta = (1 + \e^{\beta H_\Delta})^{-1}$ in \eqref{GammaDelta_definition}. Throughout this section we assume that the function $\Psi$ in the definition of $\Delta$ is in $\Hmag^1(Q_h)$. From  Lemma~\ref{Gamma_Delta_admissible}, which is proved in Section~\ref{sec:proofofadmissibility} below, we know that $\Gamma_{\Delta}$ is an admissible BCS state in this case. We define the anti-unitary operator
\begin{align*}
\Jcal &:= \begin{pmatrix} 0 & J \\ -J & 0\end{pmatrix} %, & \text{where }  \quad \begin{split} J \colon L^2(\Rbb^3) &\ra L^2(\Rbb^3), \\ f &\mapsto \ov f,\end{split}
\end{align*}
with $J$ defined below \eqref{Gamma_introduction}. The operator $H_\Delta$ obeys the relation $\Jcal H_\Delta \Jcal^* = - H_\Delta$, which implies $\Jcal\Gamma_\Delta \Jcal^* = 1 - \Gamma_\Delta$. Using this and the cyclicity of the trace, we write the entropy of $\Gamma_{\Delta}$ as
\begin{align}
S(\Gamma_\Delta) = \frac 12 \Tr[ \varphi(\Gamma_\Delta)] \label{entropy matrix},
\end{align}
where $\varphi(x) := -[x\ln(x) + (1 - x) \ln(1-x)]$ for $0 \leq x \leq 1$.
%The operator evaluated in the BCS functional is not locally trace class, in general. However, its diagonal entries are. Therefore, we need to switch to a weaker form of trace.

In order to rewrite the BCS functional, it is useful to introduce a weaker notion of trace per unit volume. More precisely, we call a gauge-periodic operator $A$ acting on $L^2(\Rbb^3)\oplus L^2(\Rbb^3)$ weakly locally trace class if $P_0AP_0$ and $Q_0AQ_0$ are locally trace class, where
\begin{align}
P_0 = \begin{pmatrix} 1 & 0 \\ 0 & 0 \end{pmatrix} \label{P0}
\end{align}
and $Q_0 = 1-P_0$, and we define its weak trace per unit volume by
\begin{align}
\Tr_0 (A):= \Tr\bigl( P_0AP_0 + Q_0 AQ_0\bigr). \label{Weak_trace_definition}
\end{align}
If an operator is locally trace class then it is also weakly locally trace class but the converse need not be true. It is true, however, in case of nonnegative operators. If an operator is locally trace class then its weak trace per unit volume and its usual trace per unit volume coincide. 

Before their appearance in the context of BCS theory in \cite{Hainzl2012,Hainzl2014}, weak traces of the above kind appeared in \cite{HLS05,FLLS11}. In \cite[Lemma 1]{HLS05} it has been shown that if two weak traces $\Tr_P$ and $\Tr_{P'}$ are defined via projections $P$ and $P'$ then $\Tr_{P}(A) = \Tr_{P'}(A)$ holds for appropriate $A$ if $P - P'$ is a Hilbert--Schmidt operator. 

% the trace is independent of the used basis, if the difference P_0-P_0’ is HS.
%
%We remark that this notion has been used earlier in the literature, see \cite{HLS05}, \cite{FLLS11}. In particular,  shows that if $P_0 - P_0'$ is locally Hilbert-Schmidt for some $P_0'$ then the sets of operators that are weakly locally trace class with respect to the analogue of \eqref{Weak_trace_definition} given by $P_0'$ and \eqref{Weak_trace_definition} itself coincide.

Let $\Gamma$ be an admissible BCS state and recall the normal state $\Gamma_0$ in \eqref{Gamma0}. 
%Writing $\alpha_\Delta(X,r)$ for the kernel of $\alpha_\Delta$, t
In terms of the weak trace per unit volume, the BCS functional can be written as
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) \hspace{-90pt}& \notag\\
%
&= \frac 12 \Tr\bigl[  (H_0\Gamma - H_0\Gamma_0) - T \varphi(\Gamma) + T \varphi(\Gamma_0)\bigr] - \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; V(r)\, |\alpha(X,r)|^2 \notag\\
%
&= \frac 12 \Tr_0\bigl[ (H_\Delta\Gamma_\Delta - H_0\Gamma_0) - T\varphi(\Gamma_\Delta) + T\varphi(\Gamma_0)\bigr] \label{kinetic energy} \\
%
&\hspace{55pt} + \frac 12 \Tr_0\bigl[ (H_\Delta \Gamma - H_\Delta \Gamma_\Delta) - T \varphi(\Gamma) + T\varphi(\Gamma_\Delta)\bigr] \label{relative_entropy_term}\\
%
&\hspace{55pt} - \frac 12 \Tr_0 \begin{pmatrix}
0 & \Delta \\ \ov \Delta & 0 \end{pmatrix} \Gamma - \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; V(r)\, |\alpha(X,r)|^2. \label{interaction-term}
\end{align}
Note that we added and subtracted the first term in \eqref{kinetic energy} and that we added and subtracted the first term in \eqref{interaction-term} to replace the Hamiltonian $H_0$ in \eqref{relative_entropy_term} by $H_\Delta$. The operators inside the traces in \eqref{kinetic energy} and \eqref{relative_entropy_term} are not necessarily locally trace class, which is the reason we introduce the weak local trace. We also note that \eqref{relative_entropy_term} equals $\frac T2$ times the relative entropy $ \Hcal_0(\Gamma, \Gamma_\Delta)$ of $\Gamma$ with respect to $\Gamma_{\Delta}$, defined in \eqref{Relative_Entropy}. 
%Furthermore, , 
%
%, recall that $\Gamma_\Delta = (1 + \e^{\beta H_\Delta})^{-1}$ and note that
%\begin{align*}
% \beta H_\Delta  +  \ln(\Gamma_\Delta) = -\ln ( \e^{-\beta H_\Delta} (1 + \e^{\beta H_\Delta})) = -\ln (1 +\e^{-\beta H_\Delta}) = \ln (1 - \Gamma_\Delta).
%\end{align*}
%This implies
%\begin{align*}
%\beta H_\Delta  + \ln(\Gamma) = \ln(1 - \Gamma_\Delta) + \ln(\Gamma) - \ln(\Gamma_\Delta).
%\end{align*}
%Inserting this into \eqref{relative_entropy}, we conclude that
%\begin{align*}
%(\beta H_\Delta  + \ln(\Gamma))\,\Gamma - (\beta H_\Delta + \ln(\Gamma_\Delta)) \, \Gamma_\Delta + (1 - \Gamma)\ln(1 - \Gamma) - (1 - \Gamma_\Delta) \ln(1 - \Gamma_\Delta) &=  \\
%%
%&\hspace{-350pt} = \Gamma\ln(1- \Gamma_\Delta)- \Gamma_\Delta\ln(1 - \Gamma_\Delta)  + \Gamma(\ln(\Gamma) - \ln(\Gamma_\Delta))\\
%%
%&\hspace{-200pt} + (1 - \Gamma) \ln(1 - \Gamma) - (1 - \Gamma_\Delta)\ln(1 - \Gamma_\Delta)\\
%%
%&\hspace{-350pt} = \Gamma (\ln(\Gamma) - \ln(\Gamma_\Delta)) + (1- \Gamma) (\ln(1 - \Gamma) - \ln(1 - \Gamma_\Delta)) = \Hcal_0(\Gamma, \Gamma_\Delta).
%\end{align*}
%

The first term in \eqref{interaction-term} can be written as
\begin{align}
-\frac  12\Tr_0 \begin{pmatrix} 0 & \Delta \\ \ov \Delta & 0\end{pmatrix} \Gamma &
%= -\frac  12\Tr_0\begin{pmatrix} \Delta \ov \alpha & \Delta (1 - \ov \gamma) \\ \ov \Delta \gamma & \ov \Delta \alpha\end{pmatrix}
=2\Re \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; (V\alpha_*)(r) \Psi(X) \; \ov \alpha(X,r). \label{additional-term}
\end{align}
The integrands in \eqref{interaction-term} and \eqref{additional-term} are equal to
\begin{equation*}
-|\alpha(X,r)|^2 + 2\Re\alpha_*(r)\Psi(X) \; \ov \alpha (X,r)  = -\bigl|\alpha(X, r) - \alpha_*(r)\Psi(X)\bigr|^2 + \bigl|\alpha_*(r)\Psi(X)\bigr|^2. 
\end{equation*}
To rewrite \eqref{kinetic energy} we need the following identities, whose proofs are straightforward computations:
\begin{align}
\Gamma_\Delta &= \frac 12 - \frac 12 \tanh\bigl( \frac \beta 2 H_\Delta\bigr), & \ln(\Gamma_\Delta) &= -\frac \beta 2 H_\Delta - \ln\bigl( 2\cosh\bigl( \frac \beta 2 H_\Delta\bigr)\bigr), \notag\\
%
1 - \Gamma_\Delta &= \frac 12 + \frac 12 \tanh\bigl( \frac\beta 2H_\Delta\bigr), & \ln(1 - \Gamma_\Delta) &= \frac\beta 2H_\Delta - \ln\bigl( 2\cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr).  \label{GammaRelations}
\end{align}
Eq.~\eqref{GammaRelations} implies
\begin{align}
\Gamma_\Delta \ln(\Gamma_\Delta) + (1-\Gamma_\Delta)\ln(1-\Gamma_\Delta) =  -\ln\bigl( 2\cosh\bigl( \frac \beta 2H_\Delta\bigr) \bigr) + \frac{\beta}{2} H_\Delta \tanh\bigl( \frac\beta 2 H_\Delta\bigr)\bigr),
\label{GammaDeltaRelation}
\end{align}
as well as
\begin{align*}
\beta H_\Delta \Gamma_\Delta - \varphi(\Gamma_\Delta) &= \frac{\beta}{2} H_\Delta - \ln \bigl( 2 \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr).
\end{align*}
This allows us to rewrite \eqref{kinetic energy} as
\begin{align}
\frac 1{2\beta}\, \Tr_0\bigl[ (\beta H_\Delta\Gamma_\Delta - \beta H_0\Gamma_0) - \varphi(\Gamma_\Delta) + \varphi(\Gamma_0)\bigr] & \notag \\
%
&\hspace{-180pt}= \frac 14 \Tr_0 \bigl[ H_\Delta - H_0\bigr] - \frac 1{2\beta}\Tr_0 \bigl[ \ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln\bigl( \cosh\bigl( \frac  \beta 2H_0\bigr)\bigr)\bigr]. \label{trace-difference-ln}
\end{align}
We note that $H_\Delta - H_0$ is weakly locally trace class and that its weak trace equals $0$. This, in particular, implies that the second term on the right side of \eqref{trace-difference-ln} is weakly locally trace class. To summarize, our intermediate result reads
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) \hspace{-60pt} & \notag\\
%
&= -\frac 1{2\beta}\Tr_0 \bigl[ \ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln\bigl( \cosh\bigl( \frac  \beta 2H_0\bigr)\bigr)\bigr] \notag\\
%
&\hspace{30pt} + \Vert\Psi \Vert_{\Lmag^2(Q_B)} \, \langle \alpha_*, V\alpha_*\rangle_{L^2(\Rbb^3)} \notag \\
%
&\hspace{30pt} +\frac{T}{2} \Hcal_0(\Gamma, \Gamma_\Delta) - \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; V(r) \, \bigl|\alpha(X,r) - \alpha_*(r)^t \Psi(X)\bigr|^2.  \label{BCS functional-intermediate}
\end{align}

In order to compute the first term on the right side of \eqref{BCS functional-intermediate}, we need Lemma~\ref{BCS functional_identity_Lemma} below. It is the main technical novelty of our trial state analysis and should be compared to the related part in the proof of \cite[Theorem~2]{Hainzl2012}. The main difference between our proof of Lemma~\ref{BCS functional_identity_Lemma} and the relevant parts of the proof of \cite[Theorem~2]{Hainzl2012} is that we use the product representation of the hyperbolic cosine in \eqref{cosh-Product} below instead of a Cauchy integral representation of the function $z \mapsto \ln(1+e^{-z})$. In this way we obtain better decay properties in the subsequent resolvent expansion, which simplifies the analysis considerably. 

As already noted above, the admissibility of $\Gamma_{\Delta}$ implies that the difference between the two operators in the first term on the right side of \eqref{BCS functional-intermediate} is weakly locally trace class. We highlight that this is a nontrivial statement because each of the two operators separately does not share this property. We also highlight that our proof of Lemma~\ref{BCS functional_identity_Lemma} does not require this as an assumption, it implies the statement independently.

In combination with \eqref{BCS functional-intermediate}, Lemma~\ref{BCS functional_identity_Lemma} below proves Proposition~\ref{BCS functional_identity}.  Before we state the lemma, we recall the definitions of the operators $L_{T, \Abold, W}$ and $N_{T, \Abold, W}$ in \eqref{LTAW_definition} and \eqref{NTAW_definition}, respectively.

%To condude the proof of , we prove in the next result, Lemma \ref{BCS functional_identity_Lemma}, that  Proposition \ref{BCS functional_identity} then follows from and Lemma \ref{BCS functional_identity_Lemma}. 

\begin{lem}
\label{BCS functional_identity_Lemma}
Let $V\alpha_*\in L^{\nicefrac 65}(\Rbb^3)\cap L^2(\Rbb^3)$. For any $B>0$, any $\Psi\in \Hmag^1(Q_B)$, and any $T>0$, the operator
\begin{align*}
\ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln \bigl( \cosh\bigl( \frac \beta 2H_0\bigr)\bigr) 
\end{align*}
is weakly locally trace class and its weak local trace equals
\begin{align}
-\frac 1{2\beta} \Tr_0\Bigl[ \ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln \bigl( \cosh\bigl( \frac \beta 2H_0\bigr)\bigr) \Bigr] & \notag\\
%
&\hspace{-140pt}= -\frac 14\langle \Delta, L_{T, \Abold, W}\Delta\rangle + \frac 18 \langle \Delta, N_{T, \Abold, W}(\Delta)\rangle + \Tr\Rcal_{T, \Abold, W}^{(1)}(\Delta). \label{BCS functional_identity_Lemma_eq2}
\end{align}
The operator $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$ is locally trace class and its trace norm satisfies the bound
\begin{align*}
\Vert \Rcal_{T, \Abold, W}^{(1)}(\Delta) \Vert_1 &\leq C\; T^{-5} \; B^3 \; \Vert \Psi\Vert_{\Hmag^1(Q_B)}^6.
\end{align*}
\end{lem}

%Proposition \ref{BCS functional_identity} now follows from \eqref{BCS functional-intermediate} and \eqref{BCS functional_identity_Lemma_eq2}. 
%Proposition \ref{BCS functional_identity_rough} is obtained by setting $\Gamma= \Gamma_\Delta$ in \eqref{BCS functional-intermediate} and combining this with \eqref{BCS functional_identity_Lemma_eq1}.

%A desirable approach for the proof of Lemma \ref{BCS functional_identity_Lemma} would be to exploit the fact that the derivative of $\ln(\cosh(x))$ equals $\tanh(x)$ and use the representation \eqref{tanh-expansion}. Since $H_\Delta$ and $H_0$ do not commute, in general, the proof is a noncommutative analogue of this idea.

\begin{proof}[Proof of Lemma \ref{BCS functional_identity_Lemma}]
We recall the Matsubara frequencies in \eqref{Matsubara_frequencies} and write the hyperbolic cosine in terms of the following product expansion, see \cite[Eq. (4.5.69)]{Handbook}, 
\begin{align}
\cosh\bigl(\frac \beta 2x\bigr) &= \prod_{k=0}^\infty \Bigl( 1 + \frac{x^2}{\omega_k^2}\Bigr). %= \prod_{k=0}^\infty \bigl( 1 + \i \, \frac{x}{\omega_k}\bigr)\bigl( 1 - \i \, \frac{x}{\omega_k}\bigr). 
\label{cosh-Product}
\end{align}
We have
\begin{align*}
0 &\leq \sum_{k= 0}^\infty \ln \bigl( 1 + \frac{x^2}{\omega_k^2}\bigr) = \ln \bigl( \cosh\bigl( \frac \beta 2 x\bigr)\bigr) \leq \frac\beta 2 \; |x|, & x &\in \Rbb,
\end{align*}
and accordingly
\begin{align*}
\ln\bigl( \cosh\bigl( \frac{\beta}{2} H_\Delta\bigr)\bigr) =  \sum_{k=0}^\infty \ln \bigl( 1+ \frac{H_\Delta^2}{\omega_k^2}\bigr) %= \sum_{k=0}^\infty \ln \bigl( 1 + \i \frac{H_\Delta}{\omega_k}\bigr) + \ln\bigl( 1 - \i \frac{H_\Delta}{\omega_k}\bigr) 
%
\end{align*}
holds in a strong sense on the domain of $|H_\Delta|$. Since $\Delta$ is a bounded operator by Lemma \ref{Schatten_estimate}, the domains of $|H_\Delta|$ and $|H_0|$ coincide. The identity 
\begin{align}
\ln\bigl( \cosh\bigl( \frac{\beta}{2} H_\Delta\bigr)\bigr) - \ln\bigl( \cosh\bigl( \frac{\beta}{2} H_0\bigr)\bigr)  =  \sum_{k=0}^\infty \bigl[ \ln \bigl( \omega_k^2+ H_\Delta^2 \bigr) - \ln \bigl( \omega_k^2 + H_0^2 \bigr) \bigr] \label{BCS functional_identity_Lemma_1}
\end{align}
therefore holds in a strong sense on the domain of $|H_0|$. Elementary arguments show that
\begin{align}
\ln\bigl( \omega^2 + H_\Delta^2\bigr) - \ln\bigl(\omega^2 + H_0^2\bigr) = -\lim_{R\to\infty} \int_\omega^R \dd u \; \Bigl[\frac{2u}{u^2 + H_\Delta^2} - \frac{2u }{u^2 + H_0^2}\Bigr] \label{ln-integral}
\end{align}
holds for $\omega>0$ in a strong sense on the domain of $\ln(1+|H_0|)$. Therefore, by \eqref{BCS functional_identity_Lemma_1} and \eqref{ln-integral}, we have
%We claim that the integral on the right side also converges in the norm topology of $\Scal^\infty$, which, in particular implies that the operator on the left side is a bounded. To see this, we intend to show that the right side of \eqref{ln-integral} is a Cauchy sequence The limit of the operator on the right side exists in .
\begin{align}
\ln\bigl( \cosh\bigl(\frac \beta 2 H_\Delta\bigr)\bigr) - \ln\bigl( \cosh\bigl( \frac \beta 2 H_0\bigr)\bigr) & \notag \\
%
&\hspace{-100pt}= -\i \sum_{k=0}^\infty \int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_\Delta } - \frac{1}{\i u - H_0} + \frac{1}{\i u + H_\Delta} - \frac{1}{\i u + H_0}\Bigr] \label{lncosh-difference}
\end{align}
in a strong sense on the domain of $|H_0|$. By a slight abuse of notation, we have incorporated the limit in \eqref{ln-integral} into the integral.
%Here the integral $\int_{\omega_k}^\infty$ has to be understood as the limit in \eqref{ln-integral}.
%
%
%
%
%
%Since $\frac \dd\dx \ln(\cosh(x)) = \tanh(x)$, we may write
%\begin{align}
%\ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln \bigl( \cosh\bigl( \frac \beta 2H_0\bigr)\bigr)  &= \frac \beta 2 \int_0^1 \dt \; \tanh\bigl( \frac\beta 2H_{t\Delta} \bigr) \; \begin{pmatrix} 0 & \Delta \\ \ov \Delta & 0\end{pmatrix} \label{Trace_Class_1}.
%\end{align}
%Applying the expansion of $\tanh$ \eqref{tanh-expansion} with $H_\Delta$ replaced by $H_{t\Delta}$ and combining this with \eqref{Trace_Class_1}, we infer
%\begin{align*}
%\ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln \bigl( \cosh\bigl( \frac \beta 2H_0\bigr)\bigr) = \int_0^1 \dt \; \sum_{n\in \Zbb} \frac{1}{\i \omega_n - H_{t\Delta}} \begin{pmatrix} 0 & \Delta \\ \ov \Delta & 0\end{pmatrix}.
%\end{align*}
%
%
%
%
%

In the next step we use the resolvent expansion
\begin{align}
(z-H_\Delta)^{-1} = (z-H_0)^{-1} + (z-H_0)^{-1} \; (H_\Delta - H_0)\; (z-H_\Delta)^{-1} \label{Resolvent_Equation}
\end{align}
to see that the right side of \eqref{lncosh-difference} equals
\begin{align*}
\Ocal_1 + \Dcal_2 + \Ocal_3 + \Dcal_4 + \Ocal_5 - 2\beta \,  \Rcal_{T, \Abold, W}^{(1)}(\Delta),
\end{align*}
with two diagonal operators $\Dcal_2$ and $\Dcal_4$, three offdiagonal operators $\Ocal_1$, $\Ocal_3$ and $\Ocal_5$ and a remainder term $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$. The index of the operators reflects the number of $\delta$ matrices appearing in their definition. The diagonal operators $\Dcal_2$ and $\Dcal_4$ are given by
\begin{align*}
\Dcal_2 &:=  -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} + \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0} \Bigr] , \\
%
\Dcal_4 &:=  -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} \\
%
&\hspace{120pt}+ \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr]
\end{align*}
and the offdiagonal operators read
\begin{align*}
\Ocal_1 &:= -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} + \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr], \\
%
\Ocal_3 &:= -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} \\
%
&\hspace{85pt}+ \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr],\\
%
\Ocal_5 &:=  -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} \\
%
&\hspace{85pt}+ \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr].
\end{align*}
Since the operators $\Ocal_1$, $\Ocal_3$, and $\Ocal_5$ are offdiagonal, they are weakly locally trace class and their weak local trace equals $0$. We also note that the operator $\Ocal_1$ is not necessarily locally trace class, which is why we need to work with the weak local trace. The operator $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$ is defined by
\begin{align*}
\Rcal_{T, \Abold, W}^{(1)}(\Delta) & \\
%
&\hspace{-50pt}:= \frac{\i}{2\beta} \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_\Delta}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} \\
%
&\hspace{40pt}+ \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_\Delta}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr].
\end{align*}

%First, we argue that the operators $\Ocal_1$, $\Ocal_2$, and $\Ocal_3$ are indeed offdiagonal. We have
%\begin{align*}
%\frac{1}{\i u \pm H_0} \, \delta = \begin{pmatrix} \frac{1}{\i u \pm \hfrak_h} \\ & \frac{1}{\i u \mp \ov{ \hfrak_h}}
%\end{pmatrix} \begin{pmatrix} &\Delta \\ \ov \Delta \end{pmatrix} = \begin{pmatrix} & \frac{1}{\i u \pm \hfrak_h} \, \Delta \\ \frac{1}{\i u \mp \ov{\hfrak_h}}\, \ov \Delta\end{pmatrix}
%\end{align*}
%and

It remains to compute the traces of $\Dcal_2$ and $\Dcal_4$, and to estimate the trace norm of $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$. We first consider $\Dcal_2$ and use Hölder's inequality in \eqref{Schatten-Hoelder} to estimate
\begin{align}
  \Bigl\Vert \frac{1}{\i u \pm H_0} \delta \frac{1}{\i u \pm H_0} \delta \frac{1}{\i u \pm H_0}\Bigr\Vert_1 &\leq \Bigl\Vert \frac{1}{\i u \pm H_0} \Bigr\Vert_\infty^3 \; \Vert \delta\Vert_2^2 = \frac{2}{u^3} \; \Vert \Delta\Vert_2^2.
\end{align}
Therefore, Lemma \ref{Schatten_estimate} shows that the combination of series and integral defining $\Dcal_2$ converges absolutely in local trace norm.
%In combination with \eqref{Matsubara_frequencies} and an application of Lemma~\ref{Schatten_estimate}, this proves 
%\begin{equation}
%	\sum_{k=0}^\infty \int_{\omega_k}^\infty \dd u \Bigl\Vert \frac{1}{\i u \pm H_0} \delta \frac{1}{\i u \pm H_0} \delta \frac{1}{\i u \pm H_0}\Bigr\Vert_1 \leq \frac{4 \Vert \Psi \Vert_2^2}{\pi^2 T^2} \sum_{k=0}^{\infty} \frac{1}{(2k+1)^2}.
%	\label{eq:A6}
%\end{equation}
In particular, $\Dcal_2$ is locally trace class and we may arbitrarily interchange the trace with the sum and the integral to compute its trace. We do this, use the cyclicity of the trace, and obtain
\begin{equation}
\Tr \Dcal_2 =  -\i \sum_{k=0}^\infty \int_{\omega_k}^\infty \dd u \; \Tr\Bigl[\Bigl(\frac{1}{\i u - H_0}\Bigr)^2 \delta \frac{1}{\i u - H_0}\delta + \Bigl(\frac{1}{\i u + H_0}\Bigr)^2\delta \frac{1}{\i u + H_0}\delta \Bigr]. \label{eq:A7}
\end{equation}
Integration by parts shows
\begin{align*}
\int_{\omega_k}^\infty \dd u \; \Bigl(\frac{1}{\i u \pm H_0}\Bigr)^2 \delta \frac{1}{\i u \pm H_0}\delta &= -\i\; \frac{1}{\i \omega_k \pm H_0} \delta \frac{1}{\i \omega_k \pm H_0} \delta \\
%
&\hspace{80pt}- \int_{\omega_k}^\infty \dd u \; \frac{1}{\i u \pm H_0} \delta \Bigl( \frac{1}{\i u \pm H_0}\Bigr)^2 \delta,
\end{align*}
and another application of the cyclicity of the trace yields
\begin{align}
\Tr \int_{\omega_k}^\infty \dd u \; \Bigl(\frac{1}{\i u \pm H_0}\Bigr)^2 \delta \frac{1}{\i u \pm H_0}\delta &= -\frac \i 2 \; \Tr \frac{1}{\i \omega_k \pm H_0} \delta \frac{1}{\i \omega_k \pm H_0} \delta. \label{BCS functional_identity_Lemma_2}
\end{align}
Note that
\begin{align}
\frac{1}{\i \omega_k \pm H_0}\,  \delta\,  \frac{1}{\i \omega_k \pm H_0} \, \delta 
%
&= \begin{pmatrix}
\frac{1}{\i \omega_k \pm \hfrak_h} \, \Delta \frac{1}{\i \omega_k \mp \ov{\hfrak_h}} \, \ov \Delta \\ & \frac{1}{\i \omega_k \mp \ov{\hfrak_h}}\,  \ov \Delta \frac{1}{\i \omega_k \pm \hfrak_h} \, \Delta
\end{pmatrix}. \label{Calculation-entry}
\end{align}
We combine this with \eqref{eq:A7} and \eqref{BCS functional_identity_Lemma_2} and summarize the cases $\pm$ into a single sum over $n\in \Zbb$. This yields
\begin{align*}
-\frac{1}{2\beta}\Tr \Dcal_2 &= \frac{1}{2\beta}\sum_{n\in \Zbb} \Bigl\langle \Delta, \frac{1}{\i\omega_n - \hfrak_h} \Delta \frac{1}{\i\omega_n + \ov{\hfrak_h}}\Bigr\rangle =  - \frac 14\langle \Delta, L_{T, \Abold, W}\Delta\rangle,
\end{align*}
where $L_{T, \Abold, W}$ is the operator defined in \eqref{LTAW_definition}.

We argue as above to see that the integrand in the series and integral defining $\Dcal_4$ is bounded by $C \Vert \Delta\Vert_4^4 \, u^{-5}$. Moreover, we have $\Vert \Delta\Vert_4^4 \leq CB^2 \Vert V\alpha_*\Vert_{\nicefrac 43}^4 \Vert \Psi\Vert_{\Hmag^1(Q_B)}^4$ by \eqref{Magnetic_Sobolev} and Lemma \ref{Schatten_estimate}. Therefore, $\Dcal_4$ is absolutely local trace norm convergent as well. The trace of $\Dcal_4$ is computed similar to that of $\Dcal_2$. With $N_{T, \Abold, W}$ defined in \eqref{NTAW_definition}, the result reads
\begin{align}
-\frac{1}{2\beta}\Tr \Dcal_4 &= \frac 18\langle \Delta, N_{T, \Abold, W}(\Delta)\rangle. \label{NTB_size_bound_2}
\end{align} 
In case of $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$, we bound the trace norm of the operator inside the integral by $u^{-7}\Vert \Delta\Vert_6^6$. Using \eqref{Magnetic_Sobolev} and Lemma~\ref{Schatten_estimate}, we estimate the second factor by a constant times $\Vert V\alpha_*\Vert_{\nicefrac 65}^6 B^{-3}\Vert \Pi\Psi\Vert_2^6 \leq CB^3 \Vert \Psi\Vert_{\Hmag^1(Q_B)}^6$. Finally, integration over $u$ yields the term $6\pi^{-6} T^{-6} (2k+1)^{-6}$, which is summable in $k$. This proves the claimed bound for the trace norm of $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$.
\end{proof}

==> 5_Structure_of_Low-Energy_States/5.2_First_decomposition_result.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{The first decomposition result}

The proof of Theorem~\ref{Structure_of_almost_minimizers} is based on Corollary~\ref{cor:lowerbound} and is given in two steps. In the first step we drop the second term on the left side of \eqref{Lower_Bound_A_2} for a lower bound, and investigate the implications of the resulting inequality for $\alpha$. The result of the corresponding analysis is summarized in Proposition~\ref{First_Decomposition_Result} below. The second term on the left side of \eqref{Lower_Bound_A_2} is used later in Lemma~\ref{Bound_on_psi}. 

\begin{prop}
\label{First_Decomposition_Result}
Given $D_0, D_1 \geq 0 $, there is $B_0>0$ with the following properties. If, for some $0< B\leq B_0$, the wave function $\alpha\in \Lsymm$ satisfies
\begin{align}
\langle \alpha , [U^* (1-P)(1 + \pi_r^2)(1-P)U + U (1-P) (1 + \pi_r^2)(1-P)U^*] \alpha \rangle & \leq D_0 B \Vert \alpha\Vert_2^2 + D_1 B^2 , \label{First_Decomposition_Result_Assumption}
\end{align}
then there are $\Psi\in \Hmag^1(Q_B)$ and $\xi_0\in \Hsymm$ such that
\begin{align}
\alpha(X,r) =  \alpha_*(r)^t \cos\bigl( \frac r2 \cdot \Pi_X\bigr) \Psi(X) + \xi_0(X,r) \label{First_Decomposition_Result_Decomp}
\end{align}
with
\begin{align}
\langle \Psi, \Pi^2 \Psi\rangle + \Vert \xi_0\Vert_{\Hsymm}^2 \leq C\bigl( B \Vert \Psi \Vert_2^2 + D_1 B^2 \bigr).  \label{First_Decomposition_Result_Estimate}
\end{align}
%and
%\begin{align}
%C \Vert \alpha\Vert_2^2 \geq \Vert \Psi\Vert_2^2 \geq (1- C  B)\; \Vert \alpha\Vert_2^2 - CB^{\nicefrac 12}. \label{First_Decomposition_Result_Estimate_psi}
%\end{align}
\end{prop}
Before we give the proof of the a priori estimates in Proposition \ref{First_Decomposition_Result}, we define the decomposition, discuss the idea behind it, which originates from \cite{Hainzl2017}, and make the connection to other existing works. For this purpose, let the operator $A \colon \Lsymm \ra \Lmag^2(Q_B)$ be given by
\begin{align}
(A\alpha)(X) := \int_{\Rbb^3} \dd r\; \ov{\alpha_*(r)} \; \cos\bigl( \frac r2\cdot \Pi_X\bigr) \alpha(X,r). \label{Def_A}
\end{align}
A short computation shows that its adjoint $A^*\colon \Lmag^2(Q_B) \ra \Lsymm$ is given by
\begin{align}
(A^*\Psi) (X,r) = \alpha_*(r)^t \cos\bigl( \frac r2\cdot \Pi_X\bigr) \Psi(X). \label{Def_Astar}
\end{align}
We highlight that this is the form of the first term in \eqref{First_Decomposition_Result_Decomp}. For a given Cooper pair wave function $\alpha$, we use these operators to define the two functions $\Psi$ and $\xi_0$ by
\begin{align}
	\Psi &:= (AA^*)^{-1} A\alpha, & \xi_0 &:= \alpha - A^*\Psi. \label{Def_Psixi}
\end{align}
Lemma~\ref{AAstar_Positive} below guarantees that $AA^*$ is invertible, and we readily check that  \eqref{First_Decomposition_Result_Decomp} holds with these definitions. Moreover, this decomposition of $\alpha$ is orthogonal in the sense that $\langle A^* \Psi, \xi_0 \rangle = 0$ holds. The claimed orthogonality follows from
\begin{align}
	A\xi_0 =0, \label{fundamental_property}
\end{align}
which is a direct consequence of \eqref{Def_Psixi}. In the following we motivate our choice for $\Psi$ and $\xi_0$ and comment on its appearance in the literature.

The decomposition of $\alpha$ is motivated by the minimization problem for the low-energy operator $2 -UPU^* - U^*PU$, that is, the operator in \eqref{First_Decomposition_Result_Assumption} with $\pi_r^2$ replaced by zero. The operators $UPU^*$ and $U^*PU$ act as $A^*A$ on the space $\Lsymm$ of reflection symmetric functions in the relative coordinate. If $\Pi$ is replaced by $P_X$ then $A^*A$ can be written as 
\begin{equation}
	A^* A \cong \int^{\oplus}_{[0,\sqrt{ 2 \pi B}]^3} \mathrm{d}P_X \; | a_{P_X} \rangle \langle a_{P_X} |, \label{eq:directintegralA}
\end{equation}
with $| a_{P_X} \rangle \langle a_{P_X} |$ the orthogonal projection onto the function $a_{P_X}(r) = \cos(r/2 \cdot P_X) \alpha_*(r)$. Here the variable $P_X$ is the dual of the center-of-mass coordinate $X$ in the sense of Fourier transformation and $r$ denotes the relative coordinate. That is, the function $a_{P_X}(r)$ minimizes $1-A^* A$ in each fiber, whence it is the eigenfunction with respect to the lowest eigenvalue of $1 - A^* A = 1 - (UPU^* + U^*PU)/2$. This discussion should be compared to \cite[Eq. (5.47)]{Hainzl2012} and the discussion before Lemma~20 in \cite{ProceedingsSpohn}.

If $B$ is present in the magnetic momentum operator $\Pi$ the above picture changes because the components of $\Pi$ cannot be diagonalized simultaneously (they do not commute), and hence \eqref{eq:directintegralA} has no obvious equivalent in this case. The decomposition of $\alpha$ in terms of the operators $A$ and $A^*$ above has been introduced in \cite{Hainzl2017} in order to study the operator $1 - V^{\nicefrac 12} L_{T,B} V^{\nicefrac 12}$ with $L_{T,B}$ in \eqref{LTB_definition}, see also the discussion below Theorem~\ref{Calculation_of_the_GL-energy}. The situation in this work is comparable to our case with $\pi_r^2$ replaced by zero in \eqref{First_Decomposition_Result_Assumption}. Our analysis below shows that the ansatz \eqref{Def_Psixi} is useful even if the full range of energies is considered, that is, if $\pi_r^2$ is present in \eqref{First_Decomposition_Result_Assumption}. 

In the following lemma we collect useful properties of the operator $A A^*$. It should be compared to \cite[Lemma~27]{Hainzl2017}.
%
%
%
%That is, the function $f$ is the eigenfunction w.r.t. the lowest eigenvalue 
%of $1 - A^* A$, which motivates the decomposition. See also the discussion before Lemma~20 in \cite{ProceedingsSpohn} and \cite[Eq. (5.47)]{Hainzl2012}. In the case of a constant magnetic field, this reasoning is not  
%
%The above decomposition in terms of the operators $A$ and $A^*$ has been introduced in the case with a constant magnetic case in \cite{Hainzl2017}.
%
%
%The generalization of the above decomposition using the operators $A$ and $A^*$, was first introduced in \cite{Hainzl2017}. 
%We use this construction as a candidate for an approximate minimizer of the whole operator in \eqref{First_Decomposition_Result_Assumption} and set
%\begin{align}
%\Psi &:= (AA^*)^{-1} A\alpha, & \xi_0 &:= \alpha - A^*\Psi. \label{Def_Psixi}
%\end{align}
%By Lemma \ref{AAstar_Positive} below, $AA^*$ is indeed invertible. Then, \eqref{First_Decomposition_Result_Decomp} holds and the immediate and fundamental property
%\begin{align}
%A\xi_0 =0 \label{fundamental_property}
%\end{align}
%resulting from \eqref{Def_Psixi} implies that $A^*\Psi + \xi_0$ is an  orthogonal decomposition of $\alpha$ with respect to the scalar product in $\Lsymm$.

\begin{lem}
\label{AAstar_Positive}
The operators
\begin{align*}
AA^* &= \int_{\Rbb^3} \dd r\; \ov{\alpha_*(r)} \alpha_*(r)^t \cos^2\bigl( \frac{r}{2} \cdot \Pi\bigr), & 1-AA^* &= \int_{\Rbb^3} \dd r \; \ov{\alpha_*(r)} \alpha_*(r)^t \sin^2\bigl( \frac r2 \cdot \Pi\bigr) 
\end{align*}
on $\Lmag^2(Q_B)$ are both bounded nonnegative matrix-valued functions of $\Pi^2$ and satisfy the following properties:
\begin{enumerate}[(a)]
\item $0\leq AA^*\leq 1$ and $0 \leq 1 - AA^*\leq 1$.
\item There is a constant $c>0$ such that $AA^* \geq c$ and $1 - AA^* \geq c \; \Pi^2\; (1 + \Pi^2)^{-1}$.
\end{enumerate}
In particular, $AA^*$ and $1 - AA^*$ are boundedly invertible on $\Lmag^2(Q_B)$.
\end{lem}

Strategy of Proof:
\begin{itemize}
\item Prove this in the ``whole-space-case'' using the spherical harmonics.
\item Use Andi's argument to lift it to the periodic case.
\end{itemize}


%\subsubsection{Proof of Lemma \ref{AAstar_Positive}}

%\begin{proof}
%Part (a) is a direct consequence of the fact that $\Vert \alpha_* \Vert_2 = 1$. In the following we reduce the proof of part (b) to known results in \cite{Hainzl2017}. To this end, we introduce the operator
%\begin{align}
%	R := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot \Pi)
%	\label{eq:R}
%\end{align}
%and note that
%\begin{align*}
%	AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R).
%\end{align*}
%Let us also denote by $\widetilde{R}$ the operator in \eqref{eq:R} but with $\Pi$ replaced by $\tilde \Pi$, which is the same operator but understood to act on $L^2(\mathbb{R}^3)$ instead of $\Lmag^2(Q_B)$. In Lemma~28 in \cite{Hainzl2017} it has been shown that $\widetilde{R}$ is a function of $\tilde \Pi^2$. Moreover, the statement of Lemma~27 in \cite{Hainzl2017} is equivalent to
%\begin{align}
%	1 - \widetilde{R}^2 \geq c\,  \frac{\tilde \Pi^2}{1 + \tilde \Pi^2}
%	\label{eq:R1}
%\end{align}
%for some $0<c<1$, and Eq.~(55) in the same reference implies
%\begin{align}
%	| \widetilde{R} | \leq 1 - c.
%	\label{eq:R2}
%\end{align}
%In combination, \eqref{eq:R1}, \eqref{eq:R2}, and $ \widetilde{R} \leq 1$ show
%\begin{align}
%	 1+\widetilde{R} &\geq c, & 1 - \widetilde{R} \geq \frac{1 - \widetilde{R}^2}{2} &\geq \frac{c}{2} \frac{\tilde \Pi^2}{1 + \tilde \Pi^2} .
%	 \label{eq:R3} 
%\end{align}
%It remains to argue that $R$ is a function of $\Pi^2$ and that a version of \eqref{eq:R3} with $\tilde R$ and $\tilde \Pi$ replaced by $R$ and $\Pi$ holds. 
%
%The fact that $R$ is a function of $\Pi^2$ follows from the argument that we used to show that the same statement is true for the operator in \eqref{eq:A29}. To show that \eqref{eq:R3} with $\tilde R$ and $\tilde \Pi$ replaced by $R$ and $\Pi$ holds, we conjugate both sides of the inequalities with the Bloch-Floquet transformation in \eqref{eq:ABF1} and \eqref{eq:ABF2}, and use \eqref{eq:ABF3}. The inequalities in \eqref{eq:R3} therefore hold equally in any fiber, that is, with $\tilde \Pi$ on the left and on the right sides replaced by $\Pi(k) = \Pi + k$ acting on $\Lmag^2(Q_B)$. Since $\tilde \Pi(0) = \Pi$, this proves the claim. 
%\end{proof}
%We note that part (a) is trivial. In contrast, part (b) needs the spectral decomposition of the operator $\Pi^2$ acting in the space $\Lmag^2(Q_B)$. In appendix \ref{Spectrum_Landau_Hamiltonian_Section}, we use a Bloch-Floquet decomposition, under which $\Pi$ fibers as a direct integral over $\vartheta\in [0,1]$ with the fiber momenta $\Pi(\vartheta) := -\i \nabla + 2\Abold + \sqrt{2\pi B} \, \vartheta \, e_3$. Proposition \ref{Spectrum_Landau_Hamiltonian} shows that the spectrum of $\Pi(\vartheta)^2$ is then given by the values $2B(2k+1) + 2\pi (p+ \vartheta)^2$ with $k\in \Nbb_0$ and $p\in \Zbb$. Moreover, there is a basis of the $k$\tho\ Landau level of the form $\{(a^*)^k |1\rangle, (a^*)^k |2\rangle\}$ with $a|1\rangle =0$ and $a|2\rangle =0$ and the well-known creation and annihilation operators in \eqref{Creation-Annihilation}.
%It fibers in the magnetic Bloch-Floquet decomposition and can be diagonalized fiberwise by using the well-known creation and annihilation operators.
%A short computation shows that, in this setting, the spectrum of $\Pi^2$ consists of the infinitely degenerate eigenvalues
%\begin{align}
%E_{k, p_3} &:= 2B (2k+1) + p_3^2 , & k &\in \Nbb_0, \; p_3\in \sqrt{2\pi B}\; \Zbb. \label{Landau_Levels}
%\end{align}


%The goal of this section is to prove Lemma \ref{AAstar_Positive}. 
%Since $\Pi$ is left invariant by the magnetic lattice translations $T_B(v)$, given by \eqref{Magnetic_Translation_Charge2}, there is a magnetic Bloch-Floquet decomposition $\Ucal_{\mathrm{BF}}$ such that the Landau Hamiltonian $\Pi^2$ fibers according to
%\begin{align*}
%\Ucal_{\mathrm{BF}} \, \Pi^2 \, \Ucal_{\mathrm{BF}}^* = \int_{Q_B^*}^\oplus \dd \vartheta \; \Pi^2(\vartheta)
%\end{align*}
%with the fiber Hamiltonians
%\begin{align*}
%\Pi^2(\vartheta) := (-\i \nabla_X + 2\Abold(X) + \vartheta)^2,
%\end{align*}
%acting on the domain $\Hmag^2(Q_B)$ for any $\vartheta\in Q_B^*$. Here, $Q_B^*$ is the fundamental cell of the dual lattice of $\Lambda_B$. We refer the interested reader to \cite[Section XIII.16]{Reedsimon4} for an introduction into Bloch-Floquet transformations and to \cite{Stefan_Peierls} for a particular treatment of the magnetic case.
%
%We claim that $\Pi^2$ can be explicitly diagonalized as a multiplication operator with the eigenvalues
%
%%Consequently, in the Bloch-Floquet representation, $\Pi^2$ becomes multiplication with the same numbers. 
%This follows from the fiberwise diagonalization of $\Pi^2(\vartheta)$ via of the well-known creation and annihilation operators built upon the magnetic momentum $\Pi + \vartheta$, and a Fourier transform in the free $X_3$-variable.
%
%The operator
%\begin{align*}
%R := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot \Pi_X)
%\end{align*}
%satisfies
%\begin{align*}
%AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R)
%\end{align*}
%and can be written as a direct integral over $\vartheta\in [0,1]$ with fiber operators
%\begin{align*}
%R(\vartheta) := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot \Pi_X(\vartheta))
%\end{align*}
%in a similar way as $\Pi^2$. Then, $R(\vartheta)$ is diagonal in the same representation used to diagonalize $\Pi(\vartheta)^2$.
%
%The proofs of Lemmas 27 and 28 in \cite{Hainzl2017} show that there is a $c >0$, independent of $\vartheta$, such that
%\begin{align*}
%R(\vartheta) &\geq - 1 + c, & R(\vartheta) &\leq 1 - c \; \frac{\Pi^2}{1 + \Pi^2}.
%\end{align*}
%From this, we easily deduce Lemma \ref{AAstar_Positive}.


%To see \eqref{Landau_Levels}, define $\Pi(\vartheta) := \Pi + \vartheta$ and let us introduce
%\begin{align*}
%a(\vartheta) &:= \frac{1}{2\sqrt{B}} \bigl( \Pi^{(1)}(\vartheta) - \i \Pi^{(2)}(\vartheta)\bigr), & a^\dagger(\vartheta) & = \frac{1}{2\sqrt{B}} \bigl( \Pi^{(1)}(\vartheta) + \i \Pi^{(2)}(\vartheta)\bigr).
%\end{align*}
%It follows that $[a(\vartheta), a^\dagger(\vartheta)] = 1$. Furthermore,
%\begin{align}
%\Pi^2(\vartheta) = 2 B \bigl( 2a^\dagger(\vartheta) a(\vartheta) + 1\bigr) + (P^{(3)} + \vartheta_3)^2. \label{AAstar_positive_3}
%\end{align}
%Here, $P^{(3)} = -\i \partial_{X_3}$ on the interval $[0,\sqrt{2\pi B^{-1}})$ with periodic boundary conditions. The operator $P^{(3)} + \vartheta_3$ can be diagonalized by the Fourier transform
%\begin{align*}
%(\Ucal_\vartheta \varphi)_m &= \frac{1}{\sqrt{2\pi B^{-1}}} \int_0^{\sqrt{2\pi B^{-1}}} \dd x_3 \; \e^{\i (\sqrt{2\pi B} \, m - \vartheta_3)x_3} \varphi(x_3) , & m &\in \Zbb,
%\end{align*} 
%having eigenvalues $p_3\in \sqrt{2\pi B}\, \Zbb$. Combining this with \eqref{AAstar_positive_3}, we read off \eqref{Landau_Levels}. 

%Consequently, \eqref{Landau_Levels} follows from taking the direct integral of $a(\vartheta)$ and $a^\dagger(\vartheta)$ over $\vartheta$. The proof shows that $\Pi^2$ can be diagonalized as well, being a multiplication operator by the numbers
%\begin{align}
%E_{k, p_3} := 2B(2k+1) + 2\pi B \; p_3^2, \qquad k\in \Nbb_0, \; p_3\in \Rbb. \label{Landau_Levels}
%\end{align}

%For the proof of Lemma \ref{AAstar_Positive}, we borrow the following auxiliary result, which is proven in \cite[Lemma 27]{Hainzl2017}. Denote the first two compontents of $\Pi$ by $\Pi^\perp = (\Pi^{(1)}, \Pi^{(2)})^t$. Moreover, by $P_{2B}^{(k)}$ we denote the projections onto the $k$\tho\ Landau level and by $L_k = L_k^{(0)}$ the Laguerre polynomials.
%
%\begin{lem}
%For every $\rho >0$,
%\begin{align*}
%\frac{1}{2\pi} \int_{\Sbb^1} \dd \omega \; \cos(\rho \omega\; \Pi^\perp) =\e^{-\frac 12 B\rho^2} \sum_{k=0}^\infty L_k(B\rho^2) P_{2B}^{(k)}.
%\end{align*}
%\end{lem}

%\begin{proof}[Proof of Lemma \ref{AAstar_Positive}]
%As noted above, part (a) is trivial. We remark that the proof of part (b) is very similar to the proof of Lemma 27 in \cite{Hainzl2017}, when $\varphi_*$ is replaced by $\alpha_*$. It actually provides the proof of Lemma \ref{AAstar_Positive} when we read it carefully enough, which we do now. Let us introduce the operator
%\begin{align*}
%R := \int_{\Rbb^3} \dd r\; \alpha_*(r)^2 \; \cos(r\cdot \Pi).
%\end{align*}
%Then, the key observation is that
%\begin{align*}
%AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R).
%\end{align*}
%
%In the representation of \eqref{Landau_Levels}, the operator $R$ is diagonalized as well, acting as a multiplication operator by the numbers
%%The operator $R$ can be diagonalized explicitly by a Fourier transform in the $x_3$ variable and decomposing into Landau levels in the $(x_1,x_2)$ variables. Then $R$ acts as a multiplication operator by the numbers
%\begin{align*}
%R_{k,p_3} &= \pi \int_0^\infty \dd u \int_\Rbb \dd x_3\; \bigl| \alpha_*\bigl( \sqrt{u + x_3^2}\bigr)\bigr|^2 \cos(x_3p_3) \e^{-\frac 12Bu} L_k(Bu), & k&\in \Nbb_0, \, p_3\in \sqrt{2\pi B} \, \Zbb.
%\end{align*}
%This formula is obtained in the same way as Eq. (49) in \cite{Hainzl2017} and $L_k$ is the $k$\tho\ Laguerre polynomial.
%
%Since $\Pi^2$ acts as multiplication by the numbers $E_{k,p_3}$ of \eqref{Landau_Levels}, it suffices to prove that there is a $c>0$ such that
%\begin{align}
%R_{k,p_3} &\geq -1 + c, & R_{k,p_3} &\leq 1 - c \frac{E_{k,p_3}}{1 + E_{k,p_3}}. \label{AAstar_positive_2}
%\end{align}
%We prove these inequalities separately for small, medium and large values of $E_{k,p_3}$. In fact, \eqref{AAstar_positive_2} is true for all $p_3\in \Rbb$.
%
%\emph{Step 1.} We claim that there are $E_* >0$ and $c_\leq , c_\geq >0$ such that for all $B>0$, $k\in\Nbb_0$ and $p_3\in \Rbb$ with $E_{k,p_3} \leq E_*$, we have
%\begin{align}
%1 - c_\leq E_{k,p_3} \leq R_{k,p_3} \leq 1 - c_\geq E_{k,p_3}. \label{AAstar_positive_1}
%\end{align}
%To see this, use $1 - \frac 12 x^2 \leq \cos x \leq 1 - \frac 12x^2 + \frac{1}{24} x^4$ for all $x\in \Rbb$ to conclude that
%\begin{align}
%0 \leq R - \int_{\Rbb^3} \dd r \; |\alpha_*(r)|^2 \bigl( 1 - \frac 12 (r\cdot \Pi)^2\bigr) \leq \frac{1}{24} \int_{\Rbb^3} \dd r \; |\alpha_*(r)|^2 (r\cdot \Pi)^4. \label{AAstar_positive_4}
%\end{align}
%Set
%\begin{align*}
%\langle |r|^{2m}\rangle &:= \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; r^{2m}, & m & = 1,2.
%\end{align*} 
%These numbers are finite by the decay properties \eqref{Decay_of_alphastar} of $\alpha_*$. An explicit computation using the fact that the angular average of $r_ir_j$ equals $\frac{1}{3} r_i^2 \delta_{ij}$ shows
%\begin{align*}
%\int_{\Rbb^3} \dd r \; \alpha_*(r)^2 (r\cdot \Pi)^2 = \frac 13 \langle |r|^2\rangle \; \Pi^2.
%\end{align*}
%Furthermore, using the operator inequality \eqref{ZPiX_inequality_quartic}, we get
%\begin{align*}
%\int_{\Rbb^3} \dd r \; \alpha_*(r)^2 (r\cdot\Pi)^4 \leq C\langle |r|^4\rangle \; (\Pi^4 + B^2).
%\end{align*}
%Combining this with \eqref{AAstar_positive_4}, we obtain
%\begin{align*}
%1 - \frac 16 \langle |r|^2\rangle \Pi^2 \leq R \leq 1 - \frac 16 \langle |r|^2 \rangle \Pi^2 + C\langle |r|^4\rangle (\Pi^4 +  B^2)
%\end{align*}
%or, equivalently,
%\begin{align*}
%1 - \frac 16 \langle |r|^2\rangle E_{k,p_3} \leq R_{k,p_3} \leq 1 - \frac 16\langle |r|^2 \rangle E_{k,p_3} + C\langle |r|^4\rangle (E_{k,p_3}^2 + B^2).
%\end{align*}
%To obtain \eqref{AAstar_positive_1} from this, we note that $B\leq E_{k,p_3}$ for every $k\in \Nbb_0$ and $p_3\in \Rbb$.
%
%Steps 2 and 3 in the proof of \cite[Lemma 28]{Hainzl2017} carry over to our situation. 
%
%\emph{Step 2} shows that $R_{k,p_3}\to 0$ as $E_{k,p_3}\to \infty$ uniformly for sufficiently small $B>0$. That is, for every $B_0>0$ and $\varepsilon>0$, there is $E_*>0$ such that for all $0\leq B\leq B_0$, all $k\in \Nbb_0$ and $p_3 \in \Rbb$ with $E_{k,p_3}\geq E_*$, we have $|R_{k,p_3}|\leq \varepsilon$.
%
%\emph{Step 3} shows that for any $E_\leq < E_\geq$ and any $B_0>0$, there is a $c>0$ such that for all $0 < B\leq B_0$, $k\in \Nbb_0$ and $p_3\in \Rbb$ with $E_\leq \leq E_{k,p_3}\leq E_\geq$, we have $|R_{k,p_3}| \leq 1 - c$.
%
%Putting the estimates together implies \eqref{AAstar_positive_2} and concludes the proof.
%\end{proof}


The remainder of this subsection is devoted to the proof of Proposition~\ref{First_Decomposition_Result}. We start with a lower bound on the operator in \eqref{First_Decomposition_Result_Assumption} when it acts on wave functions of the form $A^*\Psi$, see Lemma~\ref{MainTerm} below. 

\subsubsection{Step one -- lower bound on the range of $A^*$}

The main result of this subsection is the following lemma.

\begin{lem}
\label{MainTerm}
For any $\Psi\in \Lmag^2(Q_B)$, with $A$ and $A^*$ given by \eqref{Def_A} and \eqref{Def_Astar}, with $U$ given by \eqref{U_definition}, and $P = |\alpha_*\rangle \langle \alpha_*|$ with $\alpha_*$ from \eqref{alpha_star_ev-equation} acting on the relative coordinate, we have
\begin{align}
\frac 12 \langle A^* \Psi, [ U^* (1 - P) (1 + \pi_r^2) (1- P) U + U(1 - P) (1 + \pi_r^2)(1-P) U^* ] A^*\Psi\rangle \hspace{-340pt}& \notag\\
%
&=  \langle \Psi, AA^* (1 - AA^*)(1 + \Pi^2) \Psi\rangle \notag\\
%
&\hspace{10pt} +  \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{(1 - AA^*)\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2 \bigl(\frac r2 \Pi_X\bigr) \; (1 - AA^*)\Psi(X) \notag \\
%
&\hspace{10pt}+ \fint_{Q_B} \dd X \int_{\Rbb^3} \dr \; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2\; \sin^2 \bigl(\frac r2  \Pi_X\bigr) \; AA^*\Psi(X)\notag \\
%
&\hspace{10pt} + \frac 14 \fint_{Q_B}\dd X \int_{\Rbb^3} \dd r \; \ov{(1 - AA^*)\Psi(X)} \; |\Bbold\wedge r|^2 \alpha_*(r)^2 \; \sin^2 \bigl(\frac r2 \Pi_X\bigr) \; (1 - AA^*)\Psi(X) \notag\\
%
&\hspace{10pt} + \frac 14\fint_{Q_B}\dd X\int_{\Rbb^3} \dr \; \ov{AA^*\Psi(X)} \; |\Bbold\wedge r|^2 \alpha_*(r)^2 \;  \cos^2 \bigl(\frac r2 \Pi_X\bigr) \; AA^*\Psi(X). \label{MainTerm_5}
\end{align}
In particular, we have the lower bound
\begin{align}
\frac 12 \langle A^* \Psi, [ U^* (1 - P) (1 + \pi_r^2) (1- P) U + U(1 - P) (1 + \pi_r^2)(1-P) U^* ] A^*\Psi\rangle %& \notag\\
%
%&\hspace{-200pt}\geq \langle \Psi, AA^*(1 - AA^*)(1 + \Pi^2)\Psi\rangle
\geq c\, \langle \Psi, \Pi^2\Psi\rangle . \label{MainTerm_LowerBound}
\end{align}
\end{lem}

%By Lemma \ref{AAstar_Positive}, $AA^*$ commutes with $\Pi^2$ and the operator on the right side of \eqref{MainTerm_LowerBound} is bounded from below by a constant times $\Pi^2$. This lower bound will allow us to prove the bound on the magnetic gradient of $\Psi$ in Proposition \ref{First_Decomposition_Result}.

\begin{bem}
Let us replace $\pi_r^2$ on the left side of \eqref{MainTerm_5} by zero for the moment. In this case, the substitute of \eqref{MainTerm_5} reads
\begin{align}
\frac 12 \langle A^*\Psi, [U^*(1 - P)U + U(1 - P)U^* ] A^*\Psi\rangle = \langle \Psi , AA^*(1 - AA^*) \Psi\rangle. \label{Low_Energy_Operator}
\end{align}
It follows from Lemma~\ref{AAstar_Positive} that the operator $AA^*(1 - AA^*)$ is bounded from below by $\Pi^2$ only for small values of $\Pi^2$, which is not enough for the proof of Proposition \ref{First_Decomposition_Result}. This justifies the term ``low-energy operator'' for $1 - A^*A$, which we used earlier in the discussion below \eqref{Def_Astar}. The additional factor $1 + \Pi^2$ in the first term on the right side of \eqref{MainTerm_5} compensate for the problematic behavior of \eqref{Low_Energy_Operator} for high energies. The expression on the right side of \eqref{Low_Energy_Operator} also appears in \cite{Hainzl2017}. 
%and serves us with the appropriate bound \eqref{MainTerm_LowerBound}.
\end{bem}
%In becomes clear in the proof of Lemma \ref{MainTerm} that there is no easy way to drop any term for a lower bound until one arrives at \eqref{MainTerm_5}. Every positive term, which drops out on the way, has to account for a corresponding negative term and the network of correspondences is intricate. This is the reason why the proof of Lemma \ref{MainTerm} requires considerably more effort than \eqref{Low_Energy_Operator}.

Before we give the proof of Lemma~\ref{MainTerm}, we prove two technical lemmas, which provide intertwining relations for various magnetic momentum operators with $U$ and linear combinations of $U$. A part of the relations in the first lemma can be found in \cite[Lemma~24]{Hainzl2017}.

\begin{lem}
\label{CommutationI}
Let $p_r := -\i \nabla_r$, $\pi_r = p_r + \frac 12\Bbold \wedge r$ and $\tilde \pi_r$ and $\Pi_X$ be given by \eqref{Magnetic_Momenta_COM}. For $U$ in \eqref{U_definition}, we have the following intertwining relations:
\begin{align*}
\begin{split}
U \Pi_X U^* &= \Pi_X - \Bbold\wedge r,\phantom{\frac 12}  \\  U^* \Pi_X U &= \Pi_X + \Bbold\wedge r, \phantom{\frac 12}
\end{split} &
\begin{split}
U \pi_r U^* &= \tilde \pi_r + \frac{1}{2}\Pi_X, \\ U^* \pi_r U &= \tilde \pi_r - \frac{1}{2}\Pi_X, \phantom{\frac 12}
\end{split} &
\begin{split}
U \tilde \pi_r U^* &= p_r + \frac{1}{2}\Pi_X, \\ U^* \tilde \pi_r U &= p_r - \frac{1}{2}\Pi_X.
\end{split}
\end{align*}
\end{lem}

\begin{proof}
Let us denote $P_X := -\i \nabla_X$. We use the fact that $r\cdot P_X$ commutes with $r\cdot (\Bbold \wedge X)$ to see that
\begin{align}
U^* = \e^{\i \frac \Bbold 2 \cdot X\wedge r} \; \e^{\i \frac r2P_X} \label{representation_Ustar}
\end{align}
holds. To prove the first intertwining relation with $\Pi_X$, we compute
\begin{align*}
\Pi_XU^* &= (P_X + \Bbold\wedge X)U^* =  \e^{\i \frac \Bbold 2 \cdot X\wedge r} \Bigl[ P_X - \frac 12 \Bbold \wedge r + \Bbold\wedge X\Bigr] \e^{\i \frac r2P_X} \\
%
&= U^* \Bigl[ P_X - \frac 12 \Bbold \wedge r + \Bbold \wedge \bigl(X -\frac r2\bigr)\Bigr] = U^* [ \Pi_X - \Bbold \wedge r].
\end{align*}
Here we used that $f(X)\, \e^{\i \frac r2P_X} = \e^{\i \frac r2 P_X}\, f(X-\frac r2)$. The second intertwining relation with $\Pi_X$ is obtained by replacing $r$ by $-r$. 

Next we consider the first intertwining relation with $\pi_r$ and compute
\begin{align*}
\pi_r U^* &= \bigl( p_r + \frac 12\Bbold \wedge r\bigr) U^* = \e^{\i \frac \Bbold 2 \cdot X\wedge r}\Bigl[ p_r + (-\i)\i \frac 12 \Bbold \wedge X + \frac 12 \Bbold \wedge r\Bigr] \e^{\i \frac r2P_X} \\
%
&= U^* \Bigl[ p_r + \frac{P_X}{2} + \frac 12 \Bbold \wedge \bigl( X - \frac r2\bigr) + \frac 12 \Bbold \wedge r\Bigr] = U^* \Bigl[ \tilde \pi_r + \frac{\Pi_X}{2}\Bigr].
\end{align*}
The remaining relations can be proved similarly and we skip the details.
\end{proof}

\begin{lem}
\label{CommutationII}
\begin{enumerate}[(a)]
\item We have the following intertwining relations for $\Pi_X$:
\begin{align}
\Pi_X \cos\bigl( \frac r2 \Pi_X\bigr) &=  \cos\bigl( \frac r2 \Pi_X\bigr)\Pi_X - \i \sin\bigl( \frac r2 \Pi_X\bigr) \Bbold\wedge r, \label{PiXcos} \\
%
\Pi_X \sin\bigl( \frac r2 \Pi_X\bigr) &= \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X + \i \cos\bigl( \frac r2 \Pi_X\bigr) \Bbold\wedge r. \label{PiXsin}
\end{align}

\item The operators $p_r$, $\tilde \pi_r$ and $\pi_r$ intertwine according to
\begin{align}
\tilde \pi_r \cos\bigl( \frac r2 \Pi_X\bigr) &= \cos\bigl( \frac r2 \Pi_X\bigr) p_r + \i \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2}, \label{pirtilde_cos_pr}\\
%
\tilde \pi_r \cos\bigl( \frac r2 \Pi_X\bigr) &= \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r + \i \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr), \label{pirtilde_cos_pir}
\end{align}
and
\begin{align}
\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr)  &= \sin\bigl( \frac r2 \Pi_X\bigr) p_r - \i \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2}, \label{pirtilde_sin_pr}\\
%
\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr) &= \sin\bigl( \frac r2 \Pi_X\bigr) \pi_r - \i \frac{\Pi_X}{2} \cos\bigl( \frac r2 \Pi_X\bigr) \label{pirtilde_sin_pir}
\end{align}
\end{enumerate}
\end{lem}

It will be useful in the proof of Lemma \ref{MainTerm} to have displayed both, \eqref{pirtilde_cos_pr} and \eqref{pirtilde_cos_pir} as well as \eqref{pirtilde_sin_pr} and \eqref{pirtilde_sin_pir}, even though they follow trivially from each other and \eqref{PiXcos} or \eqref{PiXsin}.

\begin{proof}
The proof is a direct consequence of the representations
\begin{align}
	\cos\bigl( \frac r2 \Pi_X\bigr) &= \frac 12 (U^* + U), & \sin\bigl( \frac r2 \Pi_X\bigr) &= \frac 1{2\i} (U^*-U),
\end{align}
and the intertwining relations in Lemma~\ref{CommutationII}. We omit the details.
%For example, \eqref{PiXcos} is obtained from Lemma \ref{CommutationI} by computing
%\begin{align*}
%\Pi_X\cos\bigl( \frac r2 \Pi_X\bigr) &= \frac{1}{2}\Pi_X (U^* + U) = \frac{1}{2} U^* (\Pi_X - \Bbold \wedge r) + \frac{1}{2} U (\Pi_X + \Bbold \wedge r)\\
%&= \frac{1}{2} (U^* + U) \Pi_X - \frac{1}{2} (U^* - U) \Bbold \wedge r.
%\end{align*}
%Furthermore, \eqref{pirtilde_sin_pr} is obtained by
%\begin{align*}
%\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr) &= \frac{1}{2\i} U^*\bigl( p_r + \frac{\Pi_X}{2} \bigr) - \frac{1}{2\i} U \bigl( p_r - \frac{\Pi_X}{2}\bigr) = \sin\bigl( \frac r2 \Pi_X\bigr) p_r - \i \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} .
%\end{align*}
%Applying \eqref{PiXcos} to this yields \eqref{pirtilde_sin_pir}. The other equations are proved analogously.
\end{proof}

\begin{proof}[Proof of Lemma \ref{MainTerm}]
The proof is a tedious computation that is based on the intertwining relations in Lemma \ref{CommutationII}. 
%We have to keep track of the following strategy:
%\begin{enumerate}[(1)]
%\item We want to resolve the entanglement of the coordinates $X$ and $r$ that is created by the operator in \eqref{MainTerm_5}. To do this, we display every term best possible with the functions $AA^*$ and $1 - AA^*$ of $\Pi_X^2$, which we know from Lemma \ref{AAstar_Positive}. Since $A^*\Psi$ contains the operator $\cos(\frac r2\Pi_X)$, the cosine is the left-most and right-most factor in each term. Roughly speaking, we have to move it into the center in order to get $AA^*$. However, in doing so, we should never separate powers of $\Pi_X^2$, since they obviously are a function of $\Pi_X^2$ already.
%
%\item In the relative coordinate, it turns out that the natural momentum operator is the nonmagnetic $p_r = -\i \nabla_r$ and the magnetic field in $\pi_r$ should be viewed as a perturbation that leads to a positive correction in the energy. Thus, we are going to separate the magnetic field from the relative momenta.
%
%\item We make frequent use of two trivial facts. Firstly, $\Bbold \wedge r$ commutes with all of $\pi_r$, $\tilde \pi_r$, and $p_r$ because $\divv \Bbold \wedge r =0$. Secondly, $\cos( \frac r2 \Pi_X)$ and $\sin( \frac r2 \Pi_X)$ commute with any function of $r$.
%
%\item We will end up having three sorts of terms: The ones proportional to $\alpha_*^2$ having no relative magnetic field. These contribute to the main term, the first term on the right side of \eqref{MainTerm_5}. The ones proportional to $|\nabla \alpha_*|^2$ and the ones proportional to $|\Bbold\wedge r|^2\; \alpha_*^2$ are positive corrections which we are dropping later in \eqref{MainTerm_LowerBound}.
%\end{enumerate}
We start by defining
\begin{align}
\Tcal_1 &:= U^* \pi_r^2 U + U\pi_r^2 U^* = 2\, \tilde \pi_r^2 + \frac 12 \, \Pi_X^2, & \Tcal_2 &:= U^*P\pi_r^2PU + UP\pi_r^2PU^*, \notag \\
%
\Tcal_3 &:= U^* P\pi_r^2U + UP\pi_r^2U^*, & \Tcal_4 &:= U^* \pi_r^2 PU + U\pi_r^2PU^*. \label{MainTerm_6}
\end{align}
Then, \eqref{MainTerm_5} can be written as
\begin{align}
\langle A^* \Psi, [ U^* (1 - P) (1 + \pi_r^2) (1- P) U + U(1 - P) (1 + \pi_r^2)(1-P) U^* ] A^*\Psi\rangle  & = \notag\\
%
&\hspace{-330pt}= 2\langle A^*\Psi, (1 - A^*A)A^*\Psi\rangle \notag \\
%
&\hspace{-300pt} + \langle A^*\Psi, \Tcal_1 A^*\Psi\rangle + \langle A^*\Psi, \Tcal_2 A^*\Psi\rangle - \langle A^*\Psi, \Tcal_3 A^*\Psi\rangle - \langle A^*\Psi, \Tcal_4 A^*\Psi\rangle. \label{Tcal_first_line}
\end{align}
The first term on the right side equals twice the term in \eqref{Low_Energy_Operator}, which is in its final form. 

We start by computing the $\Pi_X^2$ term in $\Tcal_1$, which reads
\begin{align*}
\langle A^* \Psi , \Pi_X^2 A^* \Psi \rangle = \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \alpha^*(r) \; \cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \Psi(X).
\end{align*}
Our goal is to move $\Pi_X^2$ to the right. To that end, we apply \eqref{PiXcos} twice and obtain
\begin{align*}
\Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) = \cos\bigl( \frac r2 \Pi_X\bigr)\Pi_X^2 - \i \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X\Bbold \wedge r - \i \Pi_X \sin\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r.
\end{align*}
We multiply this from the left with $\cos( \frac r2 \Pi_X)$, use \eqref{PiXcos} to commute $\Pi_X$ to the left in the last term, and find
\begin{align}
\cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2\cos\bigl( \frac r2 \Pi_X\bigr) &= \cos^2\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 + \sin^2\bigl( \frac r2 \Pi_X\bigr) |\Bbold\wedge r|^2 \notag\\
&\hspace{-60pt}- \i \bigl[ \Pi_X\cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr) + \cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X\bigr]\Bbold\wedge r. \label{PiX-term_1}
\end{align}
The operator $| \Bbold \wedge r |^2$ in the second term on the right side commutes with $\sin^2( \frac r2 \Pi_X)$. The operator in square brackets is self-adjoint and commutes with $\Bbold \wedge r$. When we add \eqref{PiX-term_1} and its own adjoint, we obtain
%\begin{align*}
%&\hspace{-30pt}- \i \bigl[ \Pi_X\cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr) + \cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X\bigr]\Bbold\wedge r.
%\end{align*}
%We evaluate this term in the scalar product with $\alpha_*\Psi$ on both sides and make the following observations. The left-hand side is a real number. The first term on the right side equals $\langle \Psi, AA^* \Pi_X^2 \Psi\rangle$. Since $AA^*$ commutes with $\Pi_X^2$, see Lemma~\ref{AAstar_Positive}, this is a real number as well. The same is true for the second term on the right side because $|B\wedge r|$ commutes with $\sin^2(\frac r2\Pi_X)$. The operator in square brackets in the third term on the right side is self-adjoint and commutes with $\Bbold \wedge r$. In view of the $\i$ in front of the square bracket, the expectation of this term w.r.t. $\alpha_*\Psi$ is purely imaginary, and hence equals zero. This proves
\begin{align}
\cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2\cos\bigl( \frac r2 \Pi_X\bigr) & \notag\\
%
&\hspace{-50pt}= \frac 12 \cos^2\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 + \frac 12 \, \Pi_X^2 \cos^2\bigl( \frac r2 \Pi_X\bigr) + \sin^2\bigl( \frac r2 \Pi_X\bigr) |\Bbold\wedge r|^2. \label{PiX-term_2}
\end{align}
We evaluate \eqref{PiX-term_2} in the inner product with $\alpha_*\Phi$ and $\alpha_*\Psi$ on the left and right side, respectively, use the fact that $AA^*$ commutes with $\Pi^2$, see Lemma \ref{AAstar_Positive}, and obtain
\begin{align}
\langle A^*\Phi, \Pi_X^2A^*\Psi\rangle &= \langle \Phi, AA^* \Pi^2\Psi\rangle \notag\\
%
&\hspace{10pt} + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{\Phi(X)} \; |\Bbold\wedge r|^2  \alpha_*(r)^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X). \label{PiX-term}
\end{align}
When we choose $\Phi = \Psi$ we obtain the result for the term proportional to $\Pi_X^2$ in $\Tcal_1$.
%The left-hand side is a real number. The first term of the right side equals $\langle \Psi, AA^* \Pi^2 \Psi\rangle$, with $AA^*$ from Lemma \ref{AAstar_Positive}. Since $AA^*$ commutes with $\Pi^2$, this is a real number as well. As for the second term, since $|B\wedge r|$ commutes with $\sin^2(\frac r2\Pi_X)$, it is real.  In view of the $\i$ in front, the quadratic form of this term with $\alpha_*\Psi$ on both sides is a purely imaginary number and thus equal to zero. We end up with the quadratic form of the first and second term, i.e.,


Next, we investigate the term proportional to $\tilde\pi_r^2$ in $\Tcal_1$. We use \eqref{pirtilde_cos_pir} to move the operators $\tilde \pi_r$ from the middle to the outer positions and find
\begin{align}
\langle A^*\Psi, \tilde \pi_r^2A^*\Psi\rangle &= \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)} \alpha_*(r)\left[ \pi_r\cos\bigl( \frac r2 \Pi_X\bigr) -\i \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2}\right] \notag\\
%
&\hspace{80pt} \times \left[ \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r + \i \frac{\Pi_X}{2}\sin\bigl( \frac r2 \Pi_X\bigr)\right]\alpha_*(r) \Psi(X). \label{tildepir_eq1}
\end{align}
We multiply out the brackets and obtain four terms. The terms proportional to $\cos^2$ and $\sin^2$ read
\begin{align}
&\fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)}\;  |\pi_r\alpha_*(r)|^2\;  \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag\\
%
&\hspace{20pt} + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \; \alpha_*(r)\;  \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4} \sin\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \; \Psi(X).\label{tildepir_eq4}
\end{align}
For the moment the second line remains untouched. It is going to be canceled by a term in \eqref{tildepir_eq5} below. The term in the first line equals
%In the first line, we want to separate the magnetic field from $\pi_r= -\i \nabla_r + \frac 12 \Bbold \wedge r$. When we multiply out the square, the cross terms vanish because $\nabla_r\alpha_*(r)$ is proportional to $e_r$, since $\alpha_*$ is radial. Therefore, $\nabla_r\alpha_*(r) \cdot \Bbold \wedge r = 0$. Hence, the first line equals
\begin{align}
%\fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\pi_r\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) = & \notag\\
%
&\fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag \\ %\label{tildepir_eq3}\\
%
&\hspace{50pt} + \frac 14\fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X). \label{tildepir_eq2}
\end{align}
To obtain this result, we used $(\nabla \alpha_*)(r) \cdot \Bbold \wedge r =0$, which holds because $\alpha_*$ is radial. This term is in its final form.

Now we have a closer look at the terms proportional to $\sin $ times $\cos$ in \eqref{tildepir_eq1}. The operator inside the relevant quadratic form is given by
\begin{align}
\i \pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr) - \i \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r. \label{MainTerm_1}
\end{align}
We intend to interchange $\sin( \frac r2 \Pi_X)$ and $\cos( \frac r2 \Pi_X)$ in the first term. To do this, we use \eqref{PiXsin} to move $\Pi_X$ out of the center so that the first term equals
%If we move $\pi_r$ into the center afterwards, we have a cancellation. To do this, we need to move in the first term, by using . Performing this, the first term of \eqref{MainTerm_1} equals
\begin{align*}
\i \pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} -\frac 12\pi_r\cos^2\bigl( \frac r2 \Pi_X\bigr) \Bbold \wedge r.
\end{align*}
%
%Meanwhile, in the second term, we move $\pi_r$ into the center. Thus, \eqref{MainTerm_1} is equal to
%\begin{align*}
%&\pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \bigl[ \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} + \frac \i2 \cos\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r\bigr] \\
%%
%&\hspace{60pt} - \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2}\bigl[ \tilde \pi_r \cos\bigl( \frac r2 \Pi_X\bigr) - \i \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr)\bigr].
%\end{align*}
In the first term we may now commute the sine and the cosine and use \eqref{PiXcos} and \eqref{pirtilde_sin_pir} to bring $\pi_r$ and $\Pi_X$ in the center again. We also move $\pi_r$ into the center in the second term in \eqref{MainTerm_1}. As a result, \eqref{MainTerm_1} equals
\begin{align}
%\pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr) - \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r & =\\
%
&\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4}\cos\bigl( \frac r2 \Pi_X\bigr) - \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4}\sin\bigl( \frac r2 \Pi_X\bigr) \notag \\
%
&\hspace{40pt}+ \i \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{4} \sin\bigl( \frac r2 \Pi_X\bigr) \Bbold \wedge r \notag \\ %\label{MainTerm_2} \\
%
&\hspace{80pt}- \frac 12 \pi_r \cos^2\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r - \frac 12 \sin\bigl( \frac r2 \Pi_X\bigr)\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r. \label{MainTerm_3}
\end{align}
We use \eqref{pirtilde_sin_pir} to move $\tilde \pi_r$ to the left in the last term in \eqref{MainTerm_3}. One of the terms we obtain in this way cancels the third term in \eqref{MainTerm_3}. We also use $\cos( \frac r2 \Pi_X)^2 + \sin( \frac r2 \Pi_X)^2=1$ to rewrite the fourth term in \eqref{MainTerm_3}. In combination, these considerations imply that the terms in \eqref{MainTerm_3} equal
%\begin{align*}
%&\frac \i2 \pi_r \cos^2\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r + \frac \i2 \sin\bigl( \frac r2 \Pi_X\bigr)\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r \\
%%
%&\hspace{170pt} + \frac 12 \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr) \Bbold \wedge r = \frac \i2 \pi_r \Bbold \wedge r.
%\end{align*}
\begin{align}
\begin{split}
%&\pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr) - \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r = \\
%
\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4}\cos\bigl( \frac r2 \Pi_X\bigr) - \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X^2}{4}\sin\bigl( \frac r2 \Pi_X\bigr) - \frac 12 \pi_r\Bbold \wedge r. \end{split} \label{tildepir_eq5}
\end{align}
The expectation of the second term with respect to $\alpha_*(r) \Psi(X)$ cancels the second term in \eqref{tildepir_eq4}. We multiply the last term from the left and from the right with $\alpha_*(r)$, integrate over $r$ and find 
\begin{align}
\frac 12\int_{\Rbb^3} \dd r\; \alpha_*(r) \pi_r \Bbold \wedge r \alpha_*(r) = \frac 12 \int_{\Rbb^3} \ov{p_r\alpha_*(r)} \Bbold \wedge r\alpha_*(r) + \frac 14\int_{\Rbb^3} \dd r\; |\Bbold \wedge r|^2 \alpha_*(r)^2. \label{Tcal3_eq2}
\end{align}
The first term on the right side vanishes because $\alpha_*$ is radial, see the remark below \eqref{tildepir_eq4}. Let us summarize where we are. We combine \eqref{tildepir_eq1}--\eqref{Tcal3_eq2} to see that
\begin{align}
\langle A^*\Psi, \tilde \pi_r^2A^*\Psi\rangle &= \fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag \\
%
&\hspace{-30pt} + \frac 14 \fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \; \bigl( \cos^2 \bigl( \frac r2 \Pi_X\bigr) -1 \bigr) \; \Psi(X) \notag \\
%
&\hspace{-30pt} + \frac 14 \fint_{Q_B} \dd X \int_{\Rbb^3}\dd r \; \ov{\alpha_*(r) \Psi(X)} \; \cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \Psi(X). \label{eq:1}
\end{align}
The term in the last line equals $\langle A^*\Psi, \Pi_X^2A^*\Psi\rangle$ and we use \eqref{PiX-term} to rewrite it. This allows us to show 
%Namely, we investigate the last term of \eqref{tildepir_eq5}. 
%Using that $p$ commutes with $\Bbold \wedge r$, we see by integrating by parts that the first term vanishes. 
%We are left with the first term of \eqref{PiX-term}, times $\frac 14$, and the first term of \eqref{tildepir_eq2}.
%The last term cancels the magnetic fields obtained in \eqref{tildepir_eq2} and by commuting $\Pi_X^2$ through $\cos( \frac r2 \Pi_X)$, see \eqref{PiX-term}, multiplied by $\frac 14$. The remaining terms are \eqref{tildepir_eq3} and the nonmagnetic part of \eqref{PiX-term}, times $\frac 14$. 
\begin{align*}
\langle A^*\Psi, \tilde \pi_r^2A^*\Psi\rangle &= \frac 14 \langle \Psi, AA^* \Pi^2\Psi\rangle + \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\;  \ov{\Psi(X)}\;  |\nabla \alpha_*(r)|^2\;  \cos^2\bigl( \frac r2 \Pi_X\bigr)\; \Psi(X).
\end{align*}
In combination with \eqref{MainTerm_6} and \eqref{PiX-term}, this yields
\begin{align}
\langle A^* \Psi, \Tcal_1 A^*\Psi\rangle &= \langle \Psi , AA^*\Pi^2\Psi\rangle \notag \\
%
&\hspace{10pt}+ 2\fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)}\;  |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr)\;  \Psi(X) \notag \\
%
&\hspace{10pt} + \frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \; |\Bbold\wedge r|^2 \alpha_*(r)^2\; \sin^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X)  \label{Tcal1-Result}
\end{align}
and completes our computation of the term involving $\Tcal_1$.

A short computation shows that
\begin{equation}
\langle A^*\Psi , \Tcal_2A^*\Psi\rangle = 2\, \langle AA^*\Psi , AA^*\Psi\rangle \Bigl[ \Vert \nabla \alpha_*\Vert_2^2 + \frac 14 \int_{\Rbb^3} \dd r \; |\Bbold \wedge r|^2 \alpha_*(r)^2\Bigr]. \label{Tcal2_result}
\end{equation}
It remains to compute the terms in \eqref{Tcal_first_line} involving the operators $\Tcal_3$ and $\Tcal_4$, where $\Tcal_4^* = \Tcal_3$.
%The second equality holds because $\nabla\alpha_*(r) \cdot \Bbold \wedge r =0$, as argued below \eqref{tildepir_eq4}. 

In the following we compute the term with $\Tcal_3$. A short computation which uses the fact that $\alpha_*$ is radial shows
\begin{align}
\langle A^* \Psi, \Tcal_3A^*\Psi\rangle &= \langle \alpha_* A A^*\Psi, \pi_r^2 (U^* + U) A^*\Psi \rangle \notag\\
%
&\hspace{-30pt}= 2\fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; \ov{p_r\alpha_*(r)} \; p_r\cos^2\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \; \Psi(X) \notag\\
%
&\hspace{-10pt} + \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2\;  \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X). \label{Tcal3_eq3}
\end{align}
%Since $\alpha_*$ is radial, $p\alpha_*(r)$ is orthogonal to the unit sphere and hence also to $\Bbold \wedge r$. Thus, $\pi_r^2\alpha_*(r) = p^2\alpha_*(r) + \frac 14|\Bbold \wedge r|^2\alpha_*(r)$. 
%
%Using again that $U^*P$ and $UP$ act as $A^*\langle \alpha_*|$ on symmetric functions, 
The second term on the right side is in its final form and will be canceled by a term below. We continue with the first term, use \eqref{pirtilde_cos_pr} twice to commute $p_r$ with the squared cosine, as well as \eqref{PiXcos} and \eqref{PiXsin} to commute $\Pi_X$ to the center in the emerging terms, and find
\begin{align}
p_r\cos^2\bigl( \frac r2 \Pi_X\bigr) %&= \cos^2\bigl( \frac r2 \Pi_X\bigr)p_r + \i \cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} + \i \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr)\cos\bigl( \frac r2 \Pi_X\bigr) \notag\\
%
&= \cos^2\bigl( \frac r2 \Pi_X\bigr)p_r + \i \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X \cos\bigl( \frac r2 \Pi_X\bigr) - \frac 12 \Bbold \wedge r. \label{Tcal3_eq1}
\end{align}
We note that the last term, when inserted back into \eqref{Tcal3_eq3}, vanishes because $\alpha_*$ is radial. The first term is final and its quadratic form with $p_r \alpha_* AA^*\Psi$ and $\alpha_*\Psi$ reads
\begin{align}
2 \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2\Pi_X\bigr) \; \Psi(X). \label{MainTerm_4}
\end{align}
Let us continue with the second term on the right side of \eqref{Tcal3_eq1}. We multiply it with $p_r$ from the left and use \eqref{pirtilde_cos_pr} and \eqref{pirtilde_sin_pr} to commute $p_r$ to the right. In the two emerging terms we bring $\Pi_X$ to the center and obtain
\begin{align*}
p_r \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X\cos\bigl( \frac r2 \Pi_X\bigr) &= \sin\bigl( \frac r2 \Pi_X\bigr)\Pi_X\cos\bigl( \frac r2 \Pi_X\bigr) p_r + \i \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X^2}{2} \sin\bigl( \frac r2 \Pi_X\bigr) \\
%
&\hspace{145pt}- \i \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{2}\cos\bigl( \frac r2 \Pi_X\bigr).
\end{align*}
We plug the second term of \eqref{Tcal3_eq1}, written in this form, back into \eqref{Tcal3_eq3} and obtain
%When evaluated in the inner product with $2 AA^*\Psi\alpha_*$ and $\Psi\alpha_*$, the second term on the right side of \eqref{Tcal3_eq1} therefore reads
\begin{align}
2 \i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; \ov{p_r\alpha_*(r)} \; \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X  \cos\bigl( \frac r2 \Pi_X\bigr)\; \alpha_*(r)\; \Psi(X) \hspace{-350pt}& \notag\\
%
&= 2 \i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^* \Psi(X)} \; \alpha_*(r) \; \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X \cos\bigl( \frac r2 \Pi_X\bigr) \; p_r\alpha_*(r)\; \Psi(X) \notag \\
%
&\hspace{20pt} + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \;  \alpha_*(r) \; \cos\bigl( \frac r2 \Pi_X\bigr)\Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r)\; \Psi(X) \notag \\
%
&\hspace{20pt} - \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; \alpha_*(r) \; \sin\bigl( \frac r2 \Pi_X\bigr)\Pi_X^2 \sin\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \; \Psi(X).\label{MainTerm_7}
\end{align}
Notice that the first term on the right side equals $(-1)$ times the term on the left side. Thus, the left side equals $\frac 12$ times the third line plus the fourth line. To compute the third line of \eqref{MainTerm_7} we use \eqref{PiX-term} with the choice $\Phi = AA^*\Psi$. A short computation shows that \eqref{PiX-term_2} holds equally with $\cos$ and $\sin$ interchanged. Accordingly, $(-1)$ times the fourth line of \eqref{MainTerm_7} equals
\begin{equation*}
	\langle AA^*\Psi, (1 -AA^*) \Pi^2\Psi\rangle + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold\wedge r|^2  \alpha_*(r)^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X). 
\end{equation*}
%\begin{align}
%\sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2\sin\bigl( \frac r2 \Pi_X\bigr) &= \sin^2\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 + \cos^2\bigl( \frac r2 \Pi_X\bigr) |\Bbold\wedge r|^2 \notag\\
%%
%&\hspace{-60pt}- \i \bigl[ \Pi_X\sin\bigl( \frac r2 \Pi_X\bigr)\cos\bigl( \frac r2 \Pi_X\bigr) + \sin\bigl( \frac r2 \Pi_X\bigr)\cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X\bigr]\Bbold\wedge r, \label{MainTerm_8}
%\end{align}
In combination, these considerations imply that the left side of \eqref{MainTerm_7} is given by
%=======
%When evaluated in the inner product with $AA^*\Psi\alpha_*$ and $\Psi\alpha_*$, the second term on the right side of \eqref{Tcal3_eq1} therefore reads
%\begin{align*}
%\i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; \ov{p_r\alpha_*(r)} \; \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X  \cos\bigl( \frac r2 \Pi_X\bigr)\; \alpha_*(r)\; \Psi(X) \hspace{-350pt}&\\
%%
%&= \i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^* \Psi(X)} \; \alpha_*(r) \; \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X \cos\bigl( \frac r2 \Pi_X\bigr) \; p_r\alpha_*(r)\; \Psi(X)\\
%%
%&\hspace{20pt} - \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; \alpha_*(r) \; \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X^2}{2} \sin\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \; \Psi(X) \\
%%
%&\hspace{20pt} + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \;  \alpha_*(r) \; \cos\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X^2}{2} \cos\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r)\; \Psi(X) .
%\end{align*}
%Notice that the first term on the right side equals $(-1)$ times the term on the left side. Thus, the left side equals $\frac 12$ times the third plus fourth line. We also note that the term in the last line equals \eqref{PiX-term} with the left $\Psi$ replaced by $AA^*\Psi$. Moreover, we claim that the term in the third line equals
%>>>>>>> Stashed changes
\begin{align}
&\frac 12 \langle AA^*\Psi, AA^* \Pi^2\Psi\rangle - \frac 12 \langle AA^*\Psi, (1 -AA^*) \Pi^2\Psi\rangle \notag \\
%
&\hspace{20pt}+ \frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold\wedge r|^2  \alpha_*(r)^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X) \notag\\
%
&\hspace{20pt} - \frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold\wedge r|^2  \alpha_*(r)^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X). \label{Tcal3_eq4}
\end{align}
We note that the third term in \eqref{Tcal3_eq4} cancels the second term in \eqref{Tcal3_eq3}. Adding all this to \eqref{MainTerm_4}, we find
\begin{align}
\langle A^*\Psi, \Tcal_3 A^*\Psi\rangle &= \frac 12 \langle \Psi, AA^* AA^* \Pi^2 \Psi\rangle - \frac 12 \langle \Psi, AA^* (1 - AA^*) \Pi^2 \Psi\rangle  \notag\\
%
&\hspace{-10pt} + 2 \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag \\ 
%
&\hspace{-10pt}+ \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \;  \sin^2\bigl( \frac r2 \Pi_X\bigr)\; \Psi(X). \label{Tcal3_result}
\end{align}
The corresponding result for $\langle A^*\Psi, \Tcal_4 A^*\Psi\rangle$ is obtained by taking the complex conjugate of the right side of \eqref{Tcal3_result}, which amounts to interchanging the roles of $AA^*\Psi$ and $\Psi$ in the last two lines.

We are now prepared to collect our results and to provide the final formula for \eqref{Tcal_first_line}. We need to collect the terms in \eqref{Tcal1-Result}, \eqref{Tcal2_result}, \eqref{Tcal3_result} and the complex conjugate of \eqref{Tcal3_result}. The terms involving $|\nabla \alpha_*|^2$ read
\begin{align}
&2\fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)}\;  |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) + 2\langle AA^*\Psi, AA^*\Psi\rangle \Vert \nabla \alpha_*\Vert_2^2 \notag \\
%
&\hspace{50pt}-2 \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag \\
%
&\hspace{50pt}- 2 \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \;  AA^*\Psi(X). \label{nablaterms}
\end{align}
When we insert the factor $1 = \cos^2(\frac r2 \Pi_X) + \sin^2(\frac r2\Pi_X)$ in the second term, we obtain the final result for the terms proportional to $|\nabla \alpha_*|^2$.

%By summarizing the first two lines according to $(1 - AA^*)\Psi$, and writing
%\begin{align*}
%\langle AA^*\Psi, AA^*\Psi\rangle \Vert \nabla\alpha_*\Vert^2 &= \fint_{Q_B}\dd X\int_{\Rbb^3}\dd r \; \ov{AA^*\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X) \\
%%
%& \hspace{5pt} +\fint_{Q_B}\dd X\int_{\Rbb^3}\dd r \; \ov{AA^*\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X),
%\end{align*}
%we get that \eqref{nablaterms} is equal to
%\begin{align*}
%&2\fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{(1-AA^*)\Psi(X)}\;  |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \\
%%
%&\hspace{30pt}-2 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{(1 - AA^*)\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X) \\
%%
%&\hspace{30pt}+2\fint_{Q_B}\dd X\int_{\Rbb^3}\dd r \; \ov{AA^*\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr)\; AA^*\Psi(X).
%\end{align*}
%Summarizing the first two lines gives the final result 

The terms proportional to $\alpha_*^2$ with magnetic fields read
\begin{align*}
%\begin{split}
&\frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \; |\Bbold\wedge r|^2 \alpha_*(r)^2\; \sin^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X) \\
%
&\hspace{30pt} + \frac 12\langle AA^*\Psi, AA^*\Psi\rangle \int_{\Rbb^3} \dd r \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \\
%
&\hspace{30pt}-  \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X)  \\
%
&\hspace{30pt}-  \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \; |\Bbold \wedge r|^2\alpha_*(r)^2\; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X).%\end{split} \label{magneticterms}
\end{align*}
When we insert $1 = \cos^2(\frac r2 \Pi_X) + \sin^2(\frac r2\Pi_X)$ in the second term we can bring these terms in the claimed form.

%Summarizing the first two terms according to $(1 - AA^*)\Psi$ and writing
%\begin{align*}
%\langle AA^*\Psi, AA^*\Psi\rangle \int_{\Rbb^3} \dd r \; |\Bbold \wedge r|^2 \alpha_*(r)^2 = &\\
%%
%&\hspace{-130pt}= \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \;  |\Bbold \wedge r|^2 \alpha_*(r)^2  \; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X) \\
%%
%&\hspace{-120pt} + \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \;  |\Bbold \wedge r|^2 \alpha_*(r)^2 \;  \cos^2\bigl( \frac r2 \Pi_X\bigr)  \; AA^*\Psi(X), 
%\end{align*}
%we see that we can write \eqref{magneticterms} as
%\begin{align*}
%&\frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{(1-AA^*)\Psi(X)} \;  |\Bbold\wedge r|^2 \alpha_*(r)^2\; \sin^2\bigl( \frac r2 \Pi_X\bigr)\;  \Psi(X) \\
%%
%&\hspace{30pt} - \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{(1-AA^*)\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2  \; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X) \\
%%
%&\hspace{30pt}+ \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2  \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X).
%\end{align*}
%Combining the first two lines yields the claimed equation. 

Finally, we collect the terms proportional to $\alpha_*^2$ but without magnetic field. Taking into account the first term in \eqref{Tcal_first_line}, we find
\begin{align*}
&2\langle \Psi, AA^*(1 - AA^*)\Psi\rangle + \langle \Psi, AA^*\Pi^2\Psi\rangle + \langle \Psi, AA^*(1 - AA^*)\Pi^2\Psi\rangle - \langle \Psi, AA^* AA^* \Pi^2 \Psi\rangle \\
%
&\hspace{50pt}= 2\langle \Psi, AA^*(1 - AA^*)(1 + \Pi^2)\Psi\rangle.
\end{align*}
To obtain the result, we used that the terms coming from $\Tcal_3$ and $\Tcal_4$ are actually the same because $AA^*$ and $1 - AA^*$ commute with $\Pi^2$, see Lemma \ref{AAstar_Positive}. This proves \eqref{MainTerm_5} and the lower bound \eqref{MainTerm_LowerBound} is implied by the operator bounds in Lemma \ref{AAstar_Positive} as well.
%
%The estimate is true because the terms proportional to $|\nabla \alpha_*|^2$ and $|\Bbold \wedge r|^2\alpha_*^2$ are written in a commutative way. Hence, they are nonnegative.
\end{proof}

\subsubsection{Step two -- estimating the cross terms}

In the second step of the proof of Proposition \ref{First_Decomposition_Result} we estimate the cross terms that we obtain when the decomposition in \eqref{First_Decomposition_Result_Decomp} with $\Psi$ and $\xi_0$ in \eqref{Def_Psixi} is inserted into the left side of \eqref{First_Decomposition_Result_Assumption}. 

%Our result, that is Lemma~\ref{Decomp_Low_Momenta_Crossterms} should be compared to 
%\cite[Lemma 29]{Hainzl2017} It turns out that these can be bounded in terms of the operator $1 -A^*A$, which is the operator on the left side of \eqref{First_Decomposition_Result_Assumption}, with $\pi_r^2$ dropped for a lower bound. The result can be viewed as a low-energy estimate on $\Psi$ because the operator $AA^*(1 - AA^*)$ is bounded from below by $\Pi^2$ only for small values of $\Pi^2$, see Lemma \ref{AAstar_Positive}. Parts of Lemma \ref{Decomp_Low_Momenta_Crossterms} were already obtained in . 
%
%It turns out that these can be estimated in terms of the low-energy operator $1 - A^*A$, which we 
%This is the content of Lemma \ref{Decomp_Low_Momenta_Crossterms}. It contains a bound on $\langle \Psi, AA^*(1 - AA^*)\Psi\rangle$ and the $\Lsymm$ norm of $\xi_0$. 
%Roughly speaking, this preliminary lemma provides a low-energy estimate on $\Psi$, because the operator $AA^*(1 - AA^*)$ is bounded from below by $\Pi^2$ only for small values of $\Pi^2$, see Lemma \ref{AAstar_Positive}. However, this will be enough to bound the cross-terms that will arise when we insert the decomposition \eqref{Def_Psixi} of $\alpha$ into the operator in \eqref{First_Decomposition_Result_Assumption}.
\begin{lem}
\label{Decomp_Low_Momenta_Crossterms}
Given $D_0, D_1 \geq 0$, there is $B_0>0$ with the following properties. If, for some $0< B\leq B_0$, the wave function $\alpha\in \Lsymm$ satisfies
\begin{align*}
\frac 12 \langle \alpha , [U^* (1 - P)U + U(1 - P)U^* ]\alpha \rangle \leq D_0 B\, \Vert \alpha \Vert_2^2 + D_1B^2,
\end{align*}
then $\Psi$ and $\xi_0$ in \eqref{Def_Psixi} satisfy the estimate
\begin{align}
\langle \Psi, AA^*(1 - AA^*)\Psi\rangle + \Vert \xi_0\Vert_2^2 \leq C \bigl( B  \Vert \Psi \Vert_2^2 +D_1 B^2\bigr). \label{Estimate_Low_Momenta}
\end{align}
Furthermore, for any $\eta >0$ we have
\begin{align}
|\langle \xi_0, [U(1-P)(1+\pi_r^2)(1-P)U^* + U^* (1-P)(1+\pi_r^2)(1-P)U] A^*\Psi\rangle| & \notag \\
%
&\hspace{-180pt}\leq \eta \, \Vert \Pi\Psi\Vert^2 + C \left(1+ \eta^{-1} \right)\, \bigl( B \Vert \Psi \Vert_2^2 + D_1B^2\bigr). \label{Tcal_CrossTerms} 
\end{align}
\end{lem}

\begin{proof}
We start by noting that $A\xi_0 =0$ implies $\langle \xi_0, A^*\Psi\rangle =0$, and hence
\begin{align}
\Vert \alpha\Vert_2^2 = \Vert A^*\Psi\Vert_2^2 + \Vert \xi_0\Vert_2^2 \leq \Vert \Psi\Vert_2^2 + \Vert \xi_0\Vert_2^2. \label{Decomp_Low_Momenta_1}
\end{align}
We use $\alpha \in \Lsymm$ and $A(1 - A^*A)A^* = AA^*(1 - AA^*)$ to see that
\begin{align}
D_0 B \Vert \alpha\Vert_2^2 + D_1 B^2 &\geq \frac 12 \langle \alpha, [U^* (1 - P)U + U(1 - P)U^* ]\alpha \rangle = \langle \alpha, (1 - A^*A) \alpha\rangle \notag\\
%
&= \langle A^*\Psi, (1 - A^*A)A^*\Psi\rangle + \langle \xi_0, (1- A^*A) A^*\Psi\rangle + \langle A^*\Psi, (1- A^*A)\xi_0\rangle \notag \\
%
&\hspace{230pt} + \langle \xi_0 , (1- A^*A)\xi_0\rangle \notag \\
%
&= \langle \Psi, AA^*(1 - AA^*) \Psi\rangle + \Vert \xi_0\Vert_2^2. \label{Decomp_Low_Momenta_9}
\end{align}
From Lemma~\ref{AAstar_Positive} we know that the first term on the right side is nonnegative and hence
\begin{equation*}
	\Vert \xi_0\Vert_2^2 \leq D_0 B \Vert \alpha\Vert_2^2 + D_1 B^2.
\end{equation*}
Together with \eqref{Decomp_Low_Momenta_1}, this also proves
\begin{equation*}
(1 - D_0B)\Vert \alpha\Vert_2^2 \leq \Vert \Psi\Vert_2^2 + D_1 B^2. %\label{Bound_on_Psi_First}
\end{equation*}
Finally, this last bound \eqref{Decomp_Low_Momenta_9} prove \eqref{Estimate_Low_Momenta}.

Next we prove \eqref{Tcal_CrossTerms}. Let us define 
\begin{align}
\Tcal := U^* (1 - P)(1 + \pi_r^2)(1 - P)U + U(1 - P)(1 + \pi_r^2)(1 - P)U^* \label{Tcal_Op_Def}
\end{align}
and consider $\langle \xi_0, \Tcal A^*\Psi\rangle$. We note that $A\xi_0 =0$ implies $PU \xi_0 = 0 = PU^*\xi_0$, where the projection $P$ is understood to act on the relative coordinate. In combination with \eqref{MainTerm_6} this allows us to see that
\begin{align}
\langle \xi_0, \Tcal A^*\Psi\rangle &= \Bigl\langle \xi_0, \Bigl[2\tilde \pi_r^2 + \frac{\Pi_X^2}{2} \Bigr] A^*\Psi\Bigr\rangle - \langle \xi_0, (U^* + U) \pi_r^2 \, \alpha_* AA^*\Psi\rangle \label{Decomp_Low_Momenta_2}
\end{align}
holds. We use \eqref{PiXcos} and \eqref{PiXsin} to commute $\Pi_X^2$ in the first term on the right side of \eqref{Decomp_Low_Momenta_2} to the right and find
%\begin{align*}
%\Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) = \cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 - 2\i \sin\bigl( \frac r2 \Pi_X\bigr)\Pi_X\Bbold \wedge r  + |\Bbold\wedge r|^2\cos\bigl( \frac r2 \Pi_X\bigr).
%\end{align*}
%The above implies
\begin{align}
\frac 12\langle \xi_0, \Pi_X^2 A^*\Psi\rangle &= \frac 12\langle \xi_0, A^*\Pi_X^2\Psi\rangle \notag \\
%
&\hspace{10pt}- \i \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \sin\bigl( \frac r2 \Pi_X\bigr) \; \Bbold \wedge r\; \alpha_*(r) \; \Pi_X \Psi(X) \notag \\
%
&\hspace{10pt}+ \frac 12\fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{\xi_0(X,r)}  \; \cos\bigl( \frac r2 \Pi_X\bigr) \;  |\Bbold\wedge r|^2 \alpha_*(r) \; \Psi(X). \label{Decomp_Low_Momenta_4}
\end{align}
The first term on the right side vanishes because $A\xi_0 =0$. Similarly, we apply \eqref{pirtilde_cos_pr} and \eqref{pirtilde_sin_pr} to commute $\tilde \pi_r^2$ in the first term in \eqref{Decomp_Low_Momenta_2} to the right and find
%We obtain
%\begin{align*}
%\tilde \pi_r^2 \cos\bigl( \frac r2 \Pi_X\bigr) &= \cos\bigl( \frac r2 \Pi_X\bigr) p^2 + \i \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X p + \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4}.
%\end{align*}
%Hence,
\begin{align}
2\langle \xi_0, \tilde \pi_r^2A^*\Psi\rangle &= 2 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \cos\bigl( \frac r2 \Pi_X\bigr) \; p^2\alpha_*(r) \; \Psi(X) \notag \\ %\label{Decomp_Low_Momenta_5} \\
%
&\hspace{20pt} + 2\i \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \, \ov{\xi_0(X,r)} \;  \sin\bigl( \frac r2 \Pi_X\bigr) \; p\alpha_*(r) \; \Pi_X\Psi(X). \label{Decomp_Low_Momenta_6}
\end{align}
%Using that $\alpha_*$ is radial, $p\alpha_*(r)$ is proportional to $e_r$, whence $p\alpha_*(r)\cdot \Bbold \wedge r =0$. Therefore, 
When we combine $\pi_r^2 \alpha_*(r) = p_r^2\alpha_*(r) + \frac 14|\Bbold \wedge r|^2\alpha_*(r)$, which holds because $\alpha_*$ is radial, \eqref{Decomp_Low_Momenta_2}, \eqref{Decomp_Low_Momenta_4} and \eqref{Decomp_Low_Momenta_6}, we obtain
\begin{align*}
\langle \xi_0, \Tcal A^*\Psi\rangle &= 2 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \cos\bigl( \frac r2 \Pi_X\bigr) \; \pi_r^2\alpha_*(r) \; (1 - AA^*)\Psi(X) \\
%
&\hspace{30pt}+ 2\i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \sin\bigl( \frac r2 \Pi_X\bigr) \; \bigl[ p - \frac 12\Bbold \wedge r\bigr] \alpha_*(r) \; \Pi_X\Psi(X).
\end{align*}
Using Cauchy-Schwarz, we bound the absolute value of this by
\begin{align}
|\langle \xi_0, \Tcal A^*\Psi\rangle| \leq 2\Vert \xi_0\Vert_2 \; \bigl[ \Vert \pi_r^2\alpha_*\Vert_2 \; \Vert (1 - AA^*)\Psi\Vert_2 + \bigl(\Vert \nabla \alpha_*\Vert_2 + B \Vert \, | \cdot  |\alpha_*\Vert_2\bigr) \Vert \Pi\Psi\Vert_2\bigr], \label{Decomp_Low_Momenta_7}
\end{align}
%Since $\alpha_*$ is radial, $\Vert \pi_r^2\alpha_*\Vert_2 \leq \Vert p^2\alpha_*\Vert_2 + B \Vert \, |\cdot|^2\alpha_*\Vert_2$, so this expression is uniformly bounded in $B$ for bounded $B$. 
and with the decay properties of $\alpha_*$ in \eqref{Decay_of_alphastar} we see that the norms of $\alpha_*$ on the right side are bounded uniformly in $0 \leq B \leq B_0$. Moreover, Lemma~\ref{AAstar_Positive} and \eqref{Estimate_Low_Momenta} imply that there is a constant $c>0$ such that
\begin{equation}
	\Vert (1 - AA^*)\Psi\Vert_2^2 \leq \langle \Psi, (1-AA^*) \Psi \rangle \leq \frac{1}{c} \langle \Psi, A A^* (1-AA^*) \Psi \rangle \leq C \bigl( B  \Vert \Psi \Vert_2^2 +D_1 B^2\bigr).
\end{equation}
%Using the inequality $ab \leq \eta a^2 + \frac{1}{4\eta} b^2$ for $\eta>0$ and $a,b\geq 0$, we obtain
For $\eta >0$ we thus obtain
\begin{align}
|\langle \xi_0, \Tcal A^*\Psi\rangle| \leq C \bigl[ \eta\,  \Vert \Pi\Psi\Vert_2^2 + \eta^{-1} \, \Vert \xi_0 \Vert_2^2 + \bigl( B \Vert \Psi \Vert_2^2 +D_1 B^2\bigr) \bigr] \label{Decomp_Low_Momenta_8}
\end{align}
%By Lemma \ref{AAstar_Positive}, there is a constant $c>0$ such that
%\begin{align*}
%(1 - AA^*)^2 &\leq \frac 1c \; AA^* (1 - AA^*)^2 \leq \frac 1c \; AA^* (1- AA^*), %\label{Decomp_Low_Momenta_9}
%\end{align*}
%and $\Vert (1 - AA^*)\Psi\Vert^2 \leq \frac 1c \langle \Psi, AA^*(1 - AA^*)\Psi\rangle$. 
and an application of \eqref{Estimate_Low_Momenta} proves the claim.
\end{proof}

\subsubsection{Proof of Proposition \ref{First_Decomposition_Result}}

We recall the decomposition $\alpha = A^*\Psi + \xi_0$ with $\Psi$ and $\xi_0$ in \eqref{Def_Psixi} as well as $\Tcal$ in \eqref{Tcal_Op_Def}. From \eqref{First_Decomposition_Result_Assumption} we know that
\begin{align}
D_0 B \Vert\alpha\Vert_2^2 + D_1 B^2  \geq \langle A^*\Psi, \Tcal A^*\Psi\rangle + 2\Re\langle \xi_0, \Tcal A^*\Psi\rangle + \langle \xi_0, \Tcal\xi_0\rangle . \label{First_Decomposition_Result_1}
\end{align}
With the help of Lemma \ref{CommutationI}, the identities $PU\xi_0 = 0 = PU^*\xi_0$ imply
\begin{align}
\langle \xi_0, \Tcal \xi_0 \rangle = \Bigl\langle \xi_0, \bigl(2 + \frac{\Pi_X^2}{2} + 2\tilde \pi_r^2\bigr) \xi_0\Bigr\rangle \geq \frac 12 \, \Vert \xi_0\Vert_\Hsymm^2. \label{First_Decomposition_Result_2}
\end{align}
Lemma \ref{AAstar_Positive} guarantees the existence of a constant $\rho>0$ such that
\begin{align*}
AA^*(1 - AA^*)(1 + \Pi^2) \geq \rho\; \Pi^2.
\end{align*}
Therefore, \eqref{MainTerm_LowerBound} implies 
%that the first term of \eqref{First_Decomposition_Result_1} is bounded from below by
\begin{align}
\langle A^* \Psi, \Tcal A^*\Psi\rangle \geq 2\, \langle \Psi, AA^*(1 - AA^*) (1 + \Pi^2)\Psi\rangle \geq 2\rho\, \langle \Psi, \Pi^2\Psi\rangle. \label{First_Decomposition_Result_3}
\end{align}

To estimate the second term on the right side of \eqref{First_Decomposition_Result_1}, we note that $\Tcal$ is bounded from below by $U(1 - P)U^* + U^*(1-P)U$. Therefore, we may apply Lemma \ref{Decomp_Low_Momenta_Crossterms} with $\eta = \frac \rho2$ and find
\begin{align*}
2\Re \langle \xi_0, \Tcal A^*\Psi\rangle \geq -2\, |\langle \xi_0, \Tcal A^*\Psi\rangle| \geq - \rho \, \Vert \Pi\Psi\Vert_2^2 - C\bigl( B\Vert \Psi\Vert_2^2 + D_1 B^2\bigr).
\end{align*}
In combination with \eqref{First_Decomposition_Result_1}, \eqref{First_Decomposition_Result_2} and \eqref{First_Decomposition_Result_3}, we thus obtain
\begin{align*}
C\bigl( B\Vert \Psi\Vert_2^2 + D_1B^2 \bigr)\geq \rho \, \Vert \Pi\Psi\Vert_2^2 + \frac 12 \, \Vert \xi_0\Vert_\Hsymm^2.
\end{align*}
This proves \eqref{First_Decomposition_Result_Estimate}. %The estimate \eqref{First_Decomposition_Result_Estimate_psi} on $\Vert \Psi\Vert_2^2$ is \eqref{Bound_on_Psi_First}.

==> 5_Structure_of_Low-Energy_States/5.3_Uniform_bound_on_Psi.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Uniform estimate on \texorpdfstring{$\Vert\Psi\Vert_2$}{Psi}}

Up to now we neglected the nonlinear term on the left side of \eqref{Lower_Bound_A_2}. This term provides the inequality
\begin{align}
		\Tr\bigl[(\alpha^* \alpha)^2\bigr] \leq C \left( B \Vert \alpha\Vert_2^2 + B^2 \right). \label{Lower_Bound_A_2b}
\end{align}
In this section we will take this term and \eqref{Lower_Bound_A_2b} into account and show that it can be combined with Proposition~\ref{First_Decomposition_Result} to obtain a bound for $\Vert \Psi\Vert_2$. This will afterwards allow us to prove Theorem~\ref{Structure_of_almost_minimizers}.

\begin{lem}
\label{Bound_on_psi}
Given $D_0\geq0$, there is $B_0>0$ such that for all $0 < B \leq B_0$ the following holds. If the wave function $\alpha\in \Lsymm$ obeys \eqref{Lower_Bound_A_2} then $\Psi$ in \eqref{Def_Psixi} satisfies
\begin{align}
\Vert \Psi\Vert_2^2 &\leq CB. \label{Bound_on_psi_result}
\end{align}
\end{lem}

\begin{proof}
We recall the decomposition $\alpha = A^*\Psi + \xi_0$ with $\Psi$ and $\xi_0$ in \eqref{Def_Psixi}. Eq.~\eqref{Lower_Bound_A_2b} and an application of the triangle inequality imply
\begin{align}
C\bigl( B\Vert \Psi\Vert_2^2 + B^2\bigr)^{\nicefrac 14} \geq \Vert \alpha\Vert_4 \geq \Vert A^*\Psi\Vert_4 - \Vert \xi_0\Vert_4. \label{Nonlinearity_8}
\end{align}
Thus, it suffices to prove an upper bound for $\Vert \xi_0\Vert_4$ and a lower bound for $\Vert A^*\Psi\Vert_4$. Our proof follows closely the proof of \cite[Eq. (5.48)]{Hainzl2012}. 

\emph{Step 1.} Let us start with the upper bound on $\Vert \xi_0\Vert_4$. We claim the estimate
\begin{align}
\Vert \xi_0\Vert_4 \leq C \bigl( B^{\nicefrac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18} \Vert \Psi\Vert_2 + B^{\nicefrac 12}\bigr).
%C\bigl( B^{\nicefrac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18}\bigr) \;  \bigl(1 + B^{\nicefrac 12} \Vert \Psi\Vert_2\bigr)^{\nicefrac 12}. 
\label{Nonlinearity_1}
\end{align}
To see this, we first use Hölder's inequality to estimate $\Vert \xi_0\Vert_4^4 \leq \Vert \xi_0\Vert_2^2 \; \Vert \xi_0\Vert_\infty^2$. From Proposition~\ref{First_Decomposition_Result} we know that $\Vert \xi_0\Vert_2^2 \leq C(B\Vert \Psi\Vert_2^2+ B^2)$, and it thus remains to prove a bound for $\Vert \xi_0\Vert_\infty$. We claim that for any $\nu > 3$
\begin{align}
\Vert \xi_0\Vert_\infty \leq  1 + C_\nu\, B^{-\nicefrac 14} \, \Vert (1 + |\cdot |)^\nu \alpha_*\Vert_{\nicefrac 65} \; \Vert \Psi \Vert_6, \label{Claim_xi_infty}
\end{align}
where the right side is finite by the decay properties of $\alpha_*$ in \eqref{Decay_of_alphastar}. To prove \eqref{Claim_xi_infty}, we first note that \eqref{gamma_alpha_fermionic_relation} implies $\Vert \alpha\Vert_\infty\leq 1$, and hence $\Vert \xi_0\Vert_\infty \leq 1 + \Vert A^*\Psi\Vert_\infty$. We apply Lemma \ref{Schatten_estimate} (b) to $A^*\Psi$ and obtain \eqref{Claim_xi_infty}. We also combine \eqref{Magnetic_Sobolev} with Proposition \ref{First_Decomposition_Result} and obtain $
\Vert \Psi\Vert_6 \leq C( \Vert \Psi\Vert_2 + B^{\nicefrac 12})$. In combination, these considerations imply \eqref{Nonlinearity_1}. 

\emph{Step 2.} We claim that
\begin{align}
\Vert A^*\Psi\Vert_4^4 \geq \frac 1{16} \; \Vert \hat \alpha_* \Vert_4^4 \; \Vert \Psi\Vert_4^4 - C \bigl( B^{\nicefrac 18} \Vert \Psi\Vert_2 + B^{\nicefrac 58} \bigr)^4 \label{Nonlinearity_5}
\end{align}
holds. To prove \eqref{Nonlinearity_5}, we write $\Vert A^*\Psi\Vert_4^4 = \tr ((A^*\Psi)^* A^*\Psi)^2$. The fact that $\alpha_*$ is real-valued implies
\begin{align*}
\Vert A^*\Psi\Vert_4^4 &= \fint_{Q_B} \dd x \int_{\Rbb^3} \dd y \; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(x - z)\ov{ \left[ \cos\bigl( \frac{x - z}{2}\Pi_{\frac{x+z}{2}}\bigr)  \Psi\bigl( \frac{x+z}{2}\bigr) \right] } \mathop \times\\
%
&\hspace{150pt} \times \alpha_*(z-y) \left[ \cos\bigl( \frac{z-y}{2} \Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z+y}{2}\bigr) \right] \Bigr|^2.
\end{align*}
We use $\cos(x) = 1 - 2\sin^2(\frac x2)$ twice and find
\begin{align}
\Vert A^*\Psi\Vert_4^4 &\geq \frac 14 \Tcal_* - C \, (\Tcal_1 + \Tcal_2), \label{Nonlinearity_2}
\end{align}
where
\begin{align*}
\Tcal_* &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \;\Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(x - z) \ov{\Psi\bigl(\frac{x+z}{2}\bigr)} \alpha_*(z - y) \Psi\bigl( \frac{z+y}{2}\bigr)\Bigr|^2
\end{align*}
and 
\begin{align}
\Tcal_1 &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \;\Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(x - z) \ov{\Psi\bigl( \frac{x+z}{2}\bigr)} \mathop \times \notag\\
%
&\hspace{140pt} \times \alpha_*(z - y) \left[ \sin^2\bigl( \frac{z-y}{4} \Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z +y}{2}\bigr) \right] \Bigr|^2, \notag\\
%
\Tcal_2 &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \; \Bigl| \int_{\Rbb^3} \dd z\; \alpha_*(x - z)\ov{ \left[ \sin^2\bigl( \frac{x -z}{4} \Pi_{\frac{x+z}{2}}\bigr) \Psi\bigl( \frac{x + z}{2}\bigr) \right]} \mathop \times \notag \\
%
&\hspace{140pt} \times\alpha_*(z - y) \left[ \cos\bigl( \frac{z - y}{2}\Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z+y}{2}\bigr) \right] \Bigr|^2. \label{Nonlinearity_3}
\end{align}
In the following we derive a lower bound on $\Tcal_*$ and an upper bound on $\Tcal_1$ and $\Tcal_2$.

\emph{Lower bound on $\Tcal_*$.} We change variables $z\mapsto z + x$ and $y\mapsto y + x$ and afterwards replace $x$ by~$X$, which allows us to write
\begin{align}
\Tcal_* = \fint_{Q_B} \dd X \int_{\Rbb^3} \dy \; \Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(z) \ov{\Psi\bigl(X + \frac z2\bigr)} \alpha_*(z - y) \Psi\bigl(X + \frac{z+y}{2}\bigr)\Bigr|^2. \label{Nonlinearity_9}
\end{align}
Next, we combine $\Psi(X + \frac z2) = \e^{\i \frac z2P_X} \Psi(X)$ and the identity $\e^{\i \frac r2P_X} = \e^{\i \frac \Bbold 2 r\wedge X}\e^{\i \frac r2\Pi_X}$ in \eqref{representation_Ustar} to write $\Psi(X + \frac z2) = \e^{\i \frac \Bbold 2 z\wedge X} \e^{\i \frac z2\Pi_X} \Psi(X)$. 
%Similarly, $\Psi(X + \frac{z+y}{2}) = \e^{\i \frac{\Bbold }{2} (z+y)\wedge X} \e^{\i\frac{z+y}{2}\Pi_X}\Psi(X)$. 
We conclude that
\begin{align*}
\ov{\Psi\bigl( X + \frac z2\bigr)} \Psi\bigl(X + \frac{z+y}{2}\bigr) = \e^{\i \frac{\Bbold}{2} y\wedge X} \; \ov{\left[ \e^{\i \frac{z}{2}\Pi_X}\Psi(X) \right]} \; \left[ \e^{\i \frac{z+y}{2}\Pi_X} \Psi(X) \right],
\end{align*}
as well as
\begin{align*}
\Tcal_* = \fint_{Q_B} \dd X \int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(-z) \ov{ \left[ \e^{\i \frac z2\Pi_X} \Psi(X) \right]} \alpha_*(z - y) \left[ \e^{\i \frac{z+y}{2}\Pi_X} \Psi(X) \right] \Bigr|^2.
\end{align*}
This also implies
\begin{align}
\Tcal_* \geq \frac 14\Tcal_*^* - C(\Tcal_*^{(1)} + \Tcal_*^{(2)})
\label{eq:A1}
\end{align}
with
\begin{align*}
\Tcal_*^* := \fint_{Q_B}\dd X\int_{\Rbb^3}\dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(z)^t \ov{\Psi(X)} \alpha_*(z - y)^t \Psi(X)\Bigr|^2
\end{align*}
and
\begin{align}
\Tcal_*^{(1)} &:= \fint_{Q_B} \dd X\int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(z) \ov{\bigl[\e^{\i \frac{z}{2}\Pi_X}\Psi(X)\bigr]} \alpha_*(z - y) \bigl[\bigl( \e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X)\bigr]\Bigr|^2, \notag \\
%
\Tcal_*^{(2)} &:= \fint_{Q_B} \dd X\int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \;\alpha_*(z)  \ov{\bigl[\bigl( \e^{\i \frac z2\Pi_X} - 1\bigr) \Psi(X)\bigr]} \alpha_*(z - y) \Psi(X)\Bigr|^2. \label{Nonlinearity_10}
\end{align}
The term $\Tcal_*^*$ equals
\begin{align*}
\Tcal_*^* = \fint_{Q_B} \dd X\; |\Psi(X)|^4 \; \int_{\Rbb^3} \dd y\;\Bigl|\int_{\Rbb^3} \dd z\; \alpha_*(z)\alpha_*(y - z)\Bigr|^2 = \Vert \Psi\Vert_{L^4(Q_B)}^4 \; \Vert \alpha_* * \alpha_*\Vert_{L^2(\Rbb^3)}^2.
\end{align*}
By \eqref{Decay_of_alphastar}, the Fourier transform of $\alpha_**\alpha_*$ equals $|\hat \alpha_*|^2$. Thus, $\Vert \alpha_* *\alpha_*\Vert_2^2 = \Vert \hat \alpha_*\Vert_4^4>0$. This is the desired leading term of \eqref{Nonlinearity_5}. 

\emph{Upper bound on $\Tcal_*^{(1)}$ and $\Tcal_*^{(2)}$.} We start with $\Tcal_*^{(1)}$, expand the square and estimate
\begin{align}
&\Tcal_*^{(1)} \leq  \int_{\Rbb^3} \dd y  \int_{\Rbb^3} \dd z  \int_{\Rbb^3} \dd z' \;  | \alpha_*(z) \, \alpha_*(z') \, \alpha_*(z - y) \, \alpha_*(z' - y)| \label{Nonlinearity_13} \\
& \times \fint_{Q_B} \dd X \; \Bigl| \bigl[ \e^{\i \frac z2\Pi_X} \Psi(X) \bigr]  \bigl[ \e^{\i \frac {z'}2\Pi_X} \Psi(X) \bigr]  \bigl[ \bigl( \e^{\i \frac{z+y}{2}\Pi_X}-1\bigr) \Psi(X) \bigr]  \bigl[ \bigl( \e^{\i \frac{z'+y}{2}\Pi_X}-1\bigr) \Psi(X) \bigr] \Bigr|. \nonumber
\end{align}
When we use Hölder's inequality, \eqref{NTB-NtildeTB_3}, \eqref{ZPiX_inequality}, and \eqref{Magnetic_Sobolev} we see that the integral in the second line can be bounded by
\begin{align}
\Vert \e^{\i \frac{z}{2}\Pi} \Psi\Vert_6^2 \; \Vert (\e^{\i \frac{z+y}{2}\Pi} - 1) \Psi\Vert_6 \; \Vert (\e^{\i \frac{z+y}{2}\Pi} - 1) \Psi\Vert_2 \leq C\; \bigl|\frac{z+y}{2}\bigr| \; B^{-\nicefrac 32} \; \Vert \Pi\Psi\Vert_2^4. \label{Nonlinearity_11}
\end{align}
%
%
%
%Using Hölder in $X$, we obtain
%\begin{align*}
%\fint_{Q_B} \dd X \; |\e^{\i \frac{z}{2}\Pi_X} \Psi(X)|^2 \; \ov{\bigl(\e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X)} \; \bigl(\e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X) \leq &\\
%%
%&\hspace{-250pt} \leq \Bigl( \fint_{Q_B} \dd X \; |\e^{\i \frac z2\Pi_X} \Psi(X)|^6\Bigr)^{\nicefrac 13} \; \Bigl( \fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} - 1) \Psi(X)|^6\Bigr)^{\nicefrac 16} \mathop \times \\
%%
%&\hspace{-100pt} \times\Bigl( \fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} - 1) \Psi(X)|^2\Bigr)^{\nicefrac 12}.
%\end{align*}
%
%
%Use 
%
%
%
%For the first factor, note $|\e^{\i \frac z2\Pi_X}\Psi(X)| = |\Psi(X + \frac z2)|$, so that, since $|\Psi|$ is periodic, this term equals $\Vert \Psi\Vert_6^2$. As for the second factor.  For the last factor, we use the operator inequality \eqref{ZPiX_inequality} to obtain
%\begin{align*}
%\fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} -1)\Psi(X)|^2 &\leq \frac{|z+y|^2}{4} \; \Vert \Pi_X\Psi\Vert_2^2.
%\end{align*}
Proposition~\ref{First_Decomposition_Result} provides us with a bound for $\Vert \Pi \Psi \Vert_2$. In combination with \eqref{Nonlinearity_13}, \eqref{Nonlinearity_11}, Young's inequality, and the bound $|z + y| \leq 2|z| + |z- y|$, this implies
\begin{align}
\Tcal_*^{(1)} &\leq C \, B^{-\nicefrac 32}\,  \left( B^2 \Vert \Psi \Vert_2^4 + D_1 B^4 \right) \int_{\Rbb^3} \dd y \; \Bigl| \int_{\Rbb^3} \dd z\;  |z+y|\; |  \alpha_*(z) \alpha_*(y-z)|\Bigr|^2 \nonumber \\
&\leq C \left( B^{-\nicefrac 12} \Vert \Psi \Vert_2^4 + D_1 B^{ \nicefrac 52 } \right) \, \Vert \alpha_*\Vert_{\nicefrac 43} \, \Vert \, |\cdot|\alpha_*\Vert_{\nicefrac 43}, \label{Nonlinearity_12} 
\end{align}
where the right side is finite by \eqref{Decay_of_alphastar}. Similarly, we see that $\Tcal_*^{(2)}$ is bounded by the right side of \eqref{Nonlinearity_12}.
%\begin{align*}
%\int_{\Rbb^3} \dd z \Bigl( \int_{\Rbb^3} \dy \; \bigl| |z+y|\alpha_*(-z)\alpha_*(z-y)\bigr|^2 \Bigr)^{\nicefrac 12} \leq \sqrt{2} \Vert \alpha_*\Vert_1 \Vert |\cdot|^{\nicefrac 12}\alpha_*\Vert_2 + \Vert |\cdot|^{\nicefrac 12}\alpha_*\Vert_1 \Vert \alpha_*\Vert_2.
%\end{align*}
%All in all, we obtain a constant $0 < C < \infty$ with $\Tcal_*^{(1)} \leq C \; \Vert\Psi\Vert_6^3 \; \Vert \Pi_X\Psi\Vert_2$. Using  \eqref{Magnetic_Sobolev}, this implies the final result $\Tcal_*^{(1)} \leq C \; \Vert \Pi_X\Psi\Vert_2^4$. 
%For $\Tcal_*^{(2)}$, only \eqref{Nonlinearity_11} needs to be adjusted by the new right side $C |z| \, \Vert \Pi\Psi\Vert_2^4$. Then, \eqref{Nonlinearity_12} is estimated in the same way by $C \Vert \, |\cdot|\alpha_*\Vert_{\nicefrac 43} \Vert \alpha_*\Vert_{\nicefrac 43}$.

\emph{Upper bound on $\Tcal_1$ and $\Tcal_2$ in \eqref{Nonlinearity_3}.} Bounds for $\Tcal_1$ and $\Tcal_2$ can be obtain along the same lines as the bound for $\Tcal_*^{(1)}$. We apply the same change of variables as above and use estimates similar to the ones in \eqref{Nonlinearity_13}. In case of $\Tcal_1$, the bound in \eqref{Nonlinearity_11} needs to be replaced by
\begin{align}
\Vert \Psi\Vert_6^2 \, \bigl\Vert \sin^2\bigl( \frac{z - y}{2}  \Pi\bigr) \Psi \bigr\Vert_6 \, \bigl\Vert \sin^2\bigl( \frac{z - y}{2}  \Pi\bigr) \Psi \bigr\Vert_2 \leq C \; \frac{|z-y|}{2} \; B^{-\nicefrac 32}\,  \Vert \Pi\Psi\Vert_2^4. \label{Nonlinearity_14}
\end{align}
Here, we used $\sin^2(x) \leq |x|$ and the operator inequality in  \eqref{ZPiX_inequality} to estimate the third factor. For the first and the second factor, we used
\begin{align*}
\sin^2\bigl( \frac{z-y}{4} \Pi\bigr) = - \frac{1}{4} \bigl( 2+ \e^{\i\frac{z-y}{2} \Pi} + \e^{-\i \frac{z-y}{2}\Pi}\bigr)
\end{align*}
and \eqref{Magnetic_Sobolev} or \eqref{NTB-NtildeTB_3}, respectively. A bound for $\Tcal_2$ can be proved analogously. The final estimate we obtain in this way reads
\begin{equation}
	\Tcal_1 + \Tcal_2 \leq C \left( B^{-\nicefrac 12} \Vert \Psi \Vert_2^4 + D_1 B^{ \nicefrac 52 } \right). 
	\label{eq:A2}
\end{equation}
In combination with \eqref{Nonlinearity_2}, \eqref{eq:A1}, and \eqref{Nonlinearity_12}, this proves \eqref{Nonlinearity_5}.
%To bound $\Tcal_2$, \eqref{Nonlinearity_14} needs to be replaced by
%\begin{align*}
%\bigl\Vert \sin^2\bigl( \frac{z}{2} \Pi\bigr) \Psi \bigr\Vert_6 \, \bigl\Vert \sin^2\bigl( \frac{z}{2} \Pi\bigr) \Psi \bigr\Vert_2 \, \bigl\Vert \cos\bigl( \frac{z-y}{2} \Pi\bigr) \Psi\bigr\Vert_6^2 \leq C \; \frac{|z|}{2} \; B^{-\nicefrac 32} \, \Vert \Pi\Psi\Vert_2^4.
%\end{align*}
%Here, we used $\cos(x) = \frac 12 (\e^{\i x} + \e^{-\i x})$ and \eqref{NTB-NtildeTB_3}. Then, we obtain the bound \eqref{Nonlinearity_12} with $|z|$ instead of $|z+y|$, as for $\Tcal_*^{(2)}$.

\emph{Step 3.} We denote $c:= \frac 1{2} \Vert \hat\alpha_*\Vert_4$, insert \eqref{Nonlinearity_1} and \eqref{Nonlinearity_5} into \eqref{Nonlinearity_8} and obtain
%\begin{align*}
%C\bigl( B^{\frac 14}\Vert \Psi\Vert_2^{\nicefrac 12} + B^{\frac 18}\bigr)  &\geq  C\bigl(\Vert \Psi\Vert_2^2B + B^{\frac 12} \bigr)^{\nicefrac 14} \geq (\Vert\alpha\Vert_4^4)^{\nicefrac 14} \\
%%
%&\hspace{-80pt}\geq \bigl( c \Vert \Psi\Vert_4^4 - C( B^{\frac 12}\Vert \Psi\Vert_2 + B^{\frac 14})^4\bigr)_+^{\nicefrac 14} - C\bigl( B^{\frac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18}\bigr) (1 + B^{\nicefrac 12}\Vert \Psi\Vert_2)^{\nicefrac 12}.
%\end{align*}
%Using the inequality $(|x|^4 - |y|^4)_+^{\nicefrac 14} \geq |x| - |y|$, which can be seen by explicitly expanding the $4\tho$ power of the right side, employing $|y|\leq |x|$, we get
\begin{align}
C B^{\frac 14}\Vert \Psi\Vert_2^{\nicefrac 12}  \geq c \Vert \Psi\Vert_4 - CB^{\frac 18} \Vert \Psi\Vert_2 - CB^{\frac 12}, \label{Nonlinearity_6}
\end{align}
which holds for $B$ small enough. For $\eta >0$ the left side is bounded from above by a constant times $\eta \Vert \Psi\Vert_2 + \eta^{-1} B^{\frac 12}$ and Hölder's inequality implies $\Vert \Psi\Vert_4 \geq \Vert \Psi\Vert_2$. 
%\begin{align*}
%\Vert \Psi\Vert_{L^4(Q_B)} \geq B^{\frac 38} \; \Vert \Psi\Vert_{L^2(Q_B)}.
%\end{align*}
Accordingly,
\begin{equation}
C \left( \eta \Vert \Psi\Vert_2 + \eta^{-1} B^{\frac 12} \right) \geq (c - CB^{\frac 18}) \Vert \Psi\Vert_2 - CB^{\frac 12}.
\label{eq:A3}
\end{equation}
%Thus,
%\begin{align*}
%\geq c' B^{\frac 38} \Vert \Psi\Vert_2 - CB^{\frac 18}.
%\end{align*}\yexycolor
When we choose $\eta$ and $B$ in \eqref{eq:A3} small enough, this proves the claim.
%
%
%
%We may assume without loss that the right side is nonnnegative because if not, the proof is finished. If this is so, then we infer $\Vert \Psi\Vert_2 \geq CB^{-\nicefrac 14}$ so that
%\begin{align*}
%\Vert \Psi\Vert_2^{\nicefrac 12} &\leq C\bigl( B^{-\frac 18} + B^{-\frac 14} \; \Vert \Psi\Vert_2^{-\nicefrac 12}\bigr) \leq CB^{-\frac 18}.
%\end{align*}
%This proves the claim.
\end{proof}

==> 6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc.tex <==
%auto-ignore  % for ArXiv to process correctly



==> 6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc/6.1_BCS-energy_of_low-energy_states.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{The BCS energy of low-energy states}

In this section, we provide the lower bound on \eqref{ENERGY_ASYMPTOTICS} and the proof of Theorem~\ref{Main_Result_Tc}~(b), and thereby complete the proof of Theorems \ref{Main_Result} and \ref{Main_Result_Tc}. Let $D_1\geq 0$ and $D\in \Rbb$ be given and assume that $\Gamma$ is a gauge-periodic state at temperature $T = \Tc(1 - Dh^2)$ that satisfies \eqref{Second_Decomposition_Gamma_Assumption}. Corollary~\ref{Structure_of_almost_minimizers_corollary} provides us with a decomposition of the Cooper pair wave function $\alpha = [\Gamma]_{12}$ in terms of $\Psi_\leq$ in \eqref{PsileqPsi>_definition} and $\sigma$ in \eqref{sigma}, where $\Vert \Psi_\leq \Vert_{\Hmag^1(Q_h)} \leq C$ and where the bound
\begin{align}
	\Vert \Psi_\leq\Vert_{\Hmag^2(Q_h)}^2 &\leq C \, \varepsilon h^{-2} \, \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 \label{Lower_Bound_B_Psileq}
\end{align}
holds in terms of the function $\Psi$ in Theorem \ref{Structure_of_almost_minimizers}. 

With the function $\Psi_\leq$ we construct a Gibbs state $\Gamma_{\Delta}$ with the gap function $\Delta \equiv \Delta_{\Psi_\leq}$ as in \eqref{Delta_definition}. Using Proposition~\ref{BCS functional_identity}, we write the BCS free energy of $\Gamma$ as
\begin{align*}
	\FBCS(\Gamma) - \FBCS(\Gamma_0) &= - \frac 14 \langle \Delta, L_{T,B} \Delta\rangle + \frac 18 \langle \Delta, N_{T,B} (\Delta)\rangle + \Vert \Psi_\leq \Vert_2^2 \;  \langle \alpha_*, V\alpha_*\rangle \\
	%
	&\hspace{10pt}+ \Tr\bigl[\Rcal_{T,B}(\Delta)\bigr] + \frac T2 \Hcal_0(\Gamma, \Gamma_\Delta) - \fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; V(r) \, |\sigma(X,r)|^2,
\end{align*}
where
\begin{equation*}
	\Vert \Rcal_{T,B}(\Delta) \Vert_1 \leq C \; h^6 \; \Vert \Psi \Vert_{\Hmag^1(Q_h)}^6.
\end{equation*}
We also apply Theorem~\ref{Calculation_of_the_GL-energy} to compute the terms in the first line on the right side, and find the lower bound
\begin{align}
		\FBCS(\Gamma) - \FBCS(\Gamma_0) &\geq h^4 \; \EGL(\Psi_\leq) -C \bigl( h^5 + \varepsilon h^4 \bigr) \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 \notag \\
		%
		&\hspace{30pt}+ \frac T2 \Hcal_0(\Gamma, \Gamma_\Delta) - \fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; V(r) \, |\sigma(X,r)|^2. \label{Lower_Bound_B_2}
\end{align}
The relative entropy is nonnegative and the last term on the right side is nonpositive. In the next section we show that their sum is negligible.

==> 6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc/6.2_Relative_entropy_estimates.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Estimate on the relative entropy}

In this section we prove a lower bound for the second line in \eqref{Lower_Bound_B_2}, showing that it is negligible. 
%\begin{lem}
%For all admissible BCS states $\Gamma$, we have
%\begin{align}
%T\Hcal_0(\Gamma, \Gamma_\Delta) &\geq \Tr \Bigl[ (\Gamma - \Gamma_\Delta) \frac{H_\Delta}{\tanh(\frac \beta 2H_\Delta)} (\Gamma - \Gamma_\Delta)\Bigr]. \label{LBpartB_1}
%\end{align}
%\end{lem}
%
%\begin{proof}
%The proof is given in \cite[Lemma 5]{Hainzl2012} and uses the fact that $\Gamma_\Delta$ is admissible, which follows from Lemma \ref{Gamma_Delta_admissible}.
%\end{proof}
%
%To be able to combine the term on the right side of \eqref{LBpartB_1} and the last term on the right side of \eqref{Lower_Bound_B_2}, we first need to replace the operator $H_{\Delta}$ in the second factor on the right side of \eqref{LBpartB_1} by $H_0$. To that end, we note that the estimate $H_\Delta^2\geq (1 - \delta)H_0^2 - \delta^{-1} \Vert \Delta\Vert_\infty^2$ holds for $0 < \delta < 1$ and we rewrite it as
%\begin{align}
%H_0 \leq (1 - \delta)^{-1} \bigl( H_\Delta^2 + \delta^{-1} \Vert \Delta\Vert_\infty^2\bigr). \label{LBpartB_4}
%\end{align}
%Furthermore, we note that the series expansion 
%\begin{align*}
%	\frac{x}{\tanh(\frac x2)} = 2+ \sum_{k=1}^\infty \bigl( 2 - \frac{8k^2\pi^2}{x^2 + 4k^2\pi^2}\bigr),
%\end{align*}
%see \cite[Eq. (5.14)]{Hainzl2012}, shows that the function $x \mapsto \frac{\sqrt{x}}{\tanh(\frac \beta 2\sqrt{x})}$ is operator monotone. We use this together with \eqref{LBpartB_4} and the monotonicity of the map $x \mapsto \tanh(x)$, which yields
% \begin{align*}
%	%K_{T,B} \otimes \Idbb_{\Cbb^2}
%	\begin{pmatrix}
%		K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%	\end{pmatrix} = \frac{H_0}{\tanh(\frac \beta 2 H_0)}
%&\leq (1 - \delta)^{-\nicefrac 12} \frac{\sqrt{H_\Delta^2 + \delta^{-1}\Vert \Delta\Vert_\infty^2}}{\tanh(\frac \beta 2 \sqrt{H_\Delta^2 + \delta^{-1} \Vert\Delta\Vert_\infty^2})}.
%\end{align*}
%We may now Taylor expand this as
%\begin{align*}
%\begin{pmatrix}
%K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%\end{pmatrix} 
%&\leq (1 - \delta)^{-\nicefrac 12} \Bigl[\frac{H_\Delta}{\tanh(\frac \beta 2H_\Delta)} + \frac{\beta}{4} \int_0^{\delta^{-1} \Vert \Delta\Vert_\infty^2} \dd t \; g\bigl( \frac \beta 2 \sqrt{H_\Delta^2 + t}\bigr)\Bigr]
%\end{align*}
%with the nonnegative function 
%\begin{align*}
%g(x) &:= \frac{1}{x} \frac{1}{\tanh(x)} - \frac{1}{\tanh^2(x)} \frac{1}{\cosh^2(x)}.
%\end{align*}
%Using $\sup_{x \geq 0} g(x) \leq 1$ and $1 \leq \frac{x}{\tanh(x)}$, we conclude that
%\begin{align*}
%	%K_{T,B} \otimes \Idbb_{\Cbb^2} 
%	\begin{pmatrix}
%		K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%	\end{pmatrix} \leq (1 - \delta)^{-\nicefrac 12} \bigl( 1 +  \frac{\delta^{-1} \beta^2}{8} \;  \Vert \Delta\Vert_\infty^2\bigr) \frac{H_\Delta}{\tanh(\frac \beta 2 H_\Delta)}
%\end{align*}
%holds. We choose $\delta := \Vert \Delta\Vert_\infty$ and note that Lemma~\ref{Schatten_estimate} and \eqref{Magnetic_Sobolev} imply 
%\begin{equation}
%	\Vert \Delta\Vert_\infty \leq C \; B^{\nicefrac 14} \; \Vert \Psi \Vert_{\Hmag^1(Q_h)}.
%	\label{eq:ABDelta}
%\end{equation} 
%In particular, $\delta < 1 $ as long as $B>0$ is sufficiently small, and we have
%\begin{align}
%	\frac{H_\Delta}{\tanh(\frac \beta 2 H_\Delta)} \geq \frac{\sqrt{1 - \Vert \Delta\Vert_\infty}}{1 + \frac{\beta^2}{8} \Vert \Delta\Vert_\infty} \; \begin{pmatrix}
%		K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%	\end{pmatrix} 
%	%K_{T,B} \otimes \Idbb_{\Cbb^2} 
%	\geq (1 - C\Vert \Delta\Vert_\infty) \; \begin{pmatrix}
%		K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%	\end{pmatrix}.
%	%K_{T,B} \otimes \Idbb_{\Cbb^2}.
%	\label{LBpartB_2}
%\end{align}
%Together, \eqref{LBpartB_1} and \eqref{LBpartB_2} show
%\begin{align*}
%\frac 12 \Tr \Bigl[(\Gamma - \Gamma_\Delta)\frac{H_\Delta}{\tanh(\frac \beta 2H_\Delta)} (\Gamma - \Gamma_\Delta)\Bigr] & \\
%%
%&\hspace{-160pt} \geq (1 - C\Vert \Delta\Vert_\infty) \langle \alpha - \alpha_\Delta , K_{T,B} (\alpha - \alpha_\Delta)\rangle + (1 - C\Vert \Delta\Vert_\infty) \Tr[ (\gamma - \gamma_\Delta) K_{T,B}(\gamma - \gamma_\Delta)],
%\end{align*}
%where we can drop the last term for a lower bound because it is nonnegative if $B$ is sufficiently small. This is the lower bound for the relative entropy of $\Gamma$ with respect to $\Gamma_{\Delta}$ we were looking for. 
%
% 
%
%
%It remains to combine the first term on the right side and the interaction term on the right side of \eqref{Lower_Bound_B_2}.
To start out with, let us define the function $\eta := \alpha_* \Psi_\leq - \alpha_\Delta$. By Corollary~\ref{Structure_of_almost_minimizers_corollary} we have $\alpha - \alpha_\Delta = \sigma + \eta$ and it follows from \cite[Eqs. (6.3)-(6.7)]{DeHaSc2021} that
\begin{align}
	&\frac T2 \Hcal_0(\Gamma, \Gamma_\Delta) - \fint_{Q_h} \dd X \int_{\Rbb^3} \dd r \; V(r)|\sigma(X, r)|^2 \notag\\
	%
	%&\hspace{20pt} \geq (1 - C\Vert \Delta\Vert_\infty) \langle \sigma + \eta, K_{T,B} (\sigma + \eta)\rangle - \langle \sigma , V\sigma\rangle \notag\\
	&\hspace{20pt} \geq (1 - C\Vert \Delta\Vert_\infty) \langle \sigma, (K_{T,\Abold, W} - V) \sigma \rangle - C\Vert \Delta\Vert_\infty \Vert V\Vert_\infty \Vert \sigma \Vert_2^2 - 2 \, | \langle\eta, K_{T, \Abold, W} \sigma\rangle|. \label{Lower_Bound_2_intermediate}
\end{align}
From \eqref{KTB_Lower_bound_5} we know that the lowest eigenvalue of $K_{T, \Abold, W} - V$ is bounded from below by $-Ch^2$. Furthermore, Lemma~\ref{Schatten_estimate} and \eqref{Magnetic_Sobolev} imply 
\begin{equation}
	\Vert \Delta\Vert_\infty \leq C \; h^{\nicefrac 12} \; \Vert \Psi \Vert_{\Hmag^1(Q_h)},
	\label{eq:ABDelta}
\end{equation}
which in combination with \eqref{Second_Decomposition_sigma_estimate} implies that the first two terms on the right side of \eqref{Lower_Bound_2_intermediate} are bounded from below by 
\begin{align}
	-C \varepsilon^{-1} h^{\nicefrac 92} \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}. \label{Lower_Bound_B_3}
\end{align}
To estimate the last term on the right side of \eqref{Lower_Bound_2_intermediate}, we use \eqref{KTc_bounded_derivative} to replace $K_{T, \Abold, W}$ by $ K_{\Tc, \Abold, W}$, which yields the estimate
\begin{align*}
|\langle \eta ,(K_{T,\Abold, W} - K_{\Tc, \Abold, W} )\sigma\rangle| &\leq 2D_0 h^2 \, \Vert \sigma\Vert_2 \, \Vert \eta\Vert_2 \\
%
&\leq C \, h^6 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}.
\end{align*}
To obtain the result we also used \eqref{Second_Decomposition_sigma_estimate},  Proposition~\ref{Structure_of_alphaDelta} and \eqref{Lower_Bound_B_Psileq}. Next, we decompose $\eta = \eta_0 + \eta_\perp$ with $\eta_0(\Delta)$ and $\eta_{\perp}(\Delta)$ as in Proposition~\ref{Structure_of_alphaDelta} and write
\begin{align}
	\langle \eta, K_{\Tc, \Abold, W} \sigma \rangle &= \langle \eta_0 , K_{\Tc, \Abold, W} \sigma\rangle + \langle \eta_\perp, K_{\Tc, \Abold, W} (\sigma - \sigma_0)\rangle + \langle \eta_\perp , K_{\Tc, \Abold, W} \sigma_0\rangle. \label{Lower_Bound_B_1}
\end{align}
Using \eqref{alphaDelta_decomposition_eq2} and \eqref{Second_Decomposition_sigma_estimate}, we see that the first term on the right side of \eqref{Lower_Bound_B_1} is bounded by
\begin{align}
	|\langle \eta_0, K_{\Tc, \Abold, W} \sigma \rangle| &\leq \bigl\Vert \sqrt{K_{\Tc, \Abold, W}}\, \eta_0\bigr\Vert_{2} \bigl\Vert \sqrt{K_{\Tc, \Abold, W}}\,\sigma\bigr\Vert_{2} \notag \\
	%
	&\leq C \varepsilon^{-\nicefrac 12} h^5 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}.
	\label{eq:A30}
\end{align}
We note that $\sigma - \sigma_0 = \xi$ and use \eqref{alphaDelta_decomposition_eq3}, \eqref{Second_Decomposition_Psi_xi_estimate}, and \eqref{Lower_Bound_B_Psileq} to estimate
\begin{align}
	|\langle \eta_\perp, K_{\Tc, \Abold, W} \xi \rangle| &\leq \bigl\Vert \sqrt{K_{\Tc, \Abold, W}} \, \eta_\perp\bigr\Vert_{2} \bigl\Vert \sqrt{K_{\Tc, \Abold, W}} \, \xi \bigr\Vert_{2} \notag \\
	&\leq C\varepsilon^{\nicefrac 12} h^4 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}. \label{eq:A31} 
\end{align}
It remains to estimate the last term on the right side of \eqref{Lower_Bound_B_1}, which we write as 
\begin{align}
\langle \eta_\perp, K_{\Tc, \Abold, W} \sigma_0\rangle &= \langle \eta_\perp, K_{\Tc}^r  \sigma_0\rangle + \langle \eta_\perp, [K_{\Tc, \Abold, W}^r - K_{\Tc}^r ] \sigma_0\rangle + \langle \eta_\perp, (U-1)K_{\Tc, \Abold, W}^r \sigma_0\rangle \notag \\
%
&\hspace{170pt}  + \langle \eta_\perp, UK_{\Tc, \Abold, W}^r (U^* - 1) \sigma_0\rangle. \label{LBpartB_3}
\end{align}
with the unitary operator $U$ in \eqref{U_definition}. We recall that the operators $K_{\Tc, \Abold, W}^r$ and $K_{\Tc}^r$ act on the relative coordinate $r = x-y$. Since $\Delta(X,r) = - 2 V(r) \alpha_*(r) \Psi_{\leq}(X)$ and $\sigma_{0}(X,r) = \alpha_*(r) \Psi_>(X)$ we know from Proposition~\ref{Structure_of_alphaDelta}~(c) that the first term on the right side of \eqref{LBpartB_3} vanishes. A bound for the remaining terms is provided by the following lemma.

\begin{lem}
	\label{Lower_Bound_B_remainings}
	We have the following estimates on the remainder terms of \eqref{LBpartB_3}:
	\begin{enumerate}[(a)]
		\item $|\langle \eta_\perp, [K_{\Tc,\Abold, W}^r - K_{\Tc}^r]\sigma_0\rangle| \leq C h^6 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2$,
		
		\item $|\langle \eta_\perp, (U - 1) K_{\Tc,\Abold, W}^r  \sigma_0\rangle| \leq C \varepsilon^{\nicefrac 12} h^4 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2$,
		
		\item $|\langle \eta_\perp, UK_{\Tc, \Abold, W}^r (U^* - 1)\sigma_0\rangle| \leq C \varepsilon^{\nicefrac 12} h^4 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2$.
	\end{enumerate}
\end{lem} 

\begin{proof}
The proof for the case $W =0$ and $A =0$ is given in \cite[Lemma 6.2]{DeHaSc2021}. The extension for general $A$ and $W$ is straightforward.
\end{proof}

Accordingly, we have
\begin{align*}
|\langle \sigma, K_{T, \Abold, W} \eta \rangle | &\leq C\bigl( \varepsilon^{-\nicefrac 12} h^5 + \varepsilon^{\nicefrac 12} h^4 \bigr) \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}.
\end{align*}
We combine this with \eqref{Lower_Bound_B_2}, \eqref{Lower_Bound_2_intermediate}, and \eqref{Lower_Bound_B_3} to see that
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) & \geq h^4\, \EGL(\Psi_\leq) \notag\\
%
&\hspace{-90pt}  - C\bigl( \varepsilon^{-\nicefrac 12} h^5 + \varepsilon^{\nicefrac 12} h^4 + \varepsilon^{-1} h^{\nicefrac 92} \bigr) \Vert \Psi\Vert_{\Hmag^1(Q_h)} \bigl( \Vert \Psi\Vert_{\Hmag^1(Q_h)} + D_1 \bigr)^{\nicefrac 12}.  \label{Lower_Bound_B_8}
\end{align}
The optimal choice $\varepsilon = h^{\nicefrac 13}$ in \eqref{Lower_Bound_B_8} yields
\begin{align}
	&\FBCS(\Gamma) - \FBCS(\Gamma_0) \notag \\
	&\hspace{2cm}\geq h^4 \, \bigl(\EGL(\Psi_\leq) - C \,  h^{\nicefrac {1}{6}} \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12} \bigr). \label{Lower_Bound_B_5}
\end{align}

==> 6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc/6.3_Conclusion.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Conclusion}

We use \eqref{Lower_Bound_B_5} to complete the proofs of Theorem~\ref{Main_Result} and Theorem~\ref{Main_Result_Tc}. To prove the former, let an approximate minimizer $\Gamma$ of the BCS functional be given. This implies that \eqref{Second_Decomposition_Gamma_Assumption} holds with
\begin{align}
D_1 := \EGLGSE + \rho \label{Lower_Bound_B_4}
\end{align}
and $\rho\geq 0$. Since $\Vert \Psi\Vert_{\Hmag^1(Q_h)} \leq C$ by \eqref{Second_Decomposition_Psi_xi_estimate}, \eqref{Lower_Bound_B_5} implies
\begin{align*}
h^4 \bigl(\EGLGSE + \rho\bigr) \geq \FBCS(\Gamma) - \FBCS(\Gamma_0) \geq h^4 \bigl( \EGL(\Psi_\leq) - C\, h^{\nicefrac 16}\bigr)
\end{align*}
and this proves the remaining claims of Theorem \ref{Main_Result}.

We continue with the proof of Theorem~\ref{Main_Result_Tc}. We assume that the temperature $T$ obeys
\begin{align}
\Tc ( 1 - h^2 (\Dc - D_0 h^{\nicefrac 16})) < T \leq \Tc(1 + Ch^2), \label{TcB_Upper_Fine_1}
\end{align}
where $\Dc$ is defined in \eqref{Dc_Definition} and $D_0 > 0$. For such temperatures $T$, we claim that the BCS functional is minimized by the normal state if $D_0$ is choosen appropriately large. This concludes the proof of part (b) of Theorem \ref{Main_Result_Tc}, since Corollary \ref{TcB_First_Upper_Bound} covers the remaining temperature range.

To prove this claim, we use \eqref{Lower_Bound_B_5} as a basis and assume that \eqref{Second_Decomposition_Gamma_Assumption} holds with $D_1 =0$. For a lower bound, we may drop the nonnegative quartic term in the Ginzburg--Landau functional so that
\begin{align*}
	\EGL(\Psi_\leq) &\geq h^{-4}  \langle \Psi_\leq , (\Lambda_0 \, \Pi_\Abold^2 + \Lambda_1 \, W - Dh^2 \Lambda_2) \Psi_\leq\rangle \geq  \Lambda_2 \, ( \Dc - D) \; h^{-2} \, \Vert \Psi_\leq \Vert_2^2, 
\end{align*}
with the coefficients $\Lambda_0$, $\Lambda_1$, $\Lambda_2$, and $\Lambda_3$ in \eqref{GL-coefficient_1}-\eqref{GL_coefficient_3}, as well as $D \in \mathbb{R}$ determined by $T = \Tc(1-D h^2)$. We use the bound
\begin{align*}
\Vert \Pi \Psi\Vert_2 &\leq C \, h \, \Vert \Psi\Vert_2,
\end{align*}
whose proof is given by \cite[Eq. (5.26)]{DeHaSc2021} and combine this with \eqref{Psi>_bound} to see that
\begin{align*}
\Vert \Psi_\leq \Vert_2 \geq \Vert \Psi\Vert_2 - \Vert \Psi_>\Vert_2 \geq c \; h \; \Vert \Psi \Vert_{\Hmag^1(Q_h)} \, ( 1 - C \, h^{\nicefrac{5}{6}} ).
\label{eq:A32}
\end{align*}
We combine these observations with the lower bound \eqref{Lower_Bound_B_5} and obtain
\begin{equation}
0\geq \FBCS(\Gamma) - \FBCS(\Gamma_0) \geq c \; h^4 \; \Vert \Psi \Vert_{\Hmag^1(Q_h)}^2 \bigl( (\Dc - D)  - Ch^{\nicefrac {1}{6}}\bigr), \label{eq:A33}
\end{equation}
Since the lower bound in \eqref{TcB_Upper_Fine_1} is equivalent to
\begin{align}
\Dc - D > D_0 \, h^{\nicefrac 1{6}}, \label{TcB_Upper_Fine_2}
\end{align}
the choice $D_0 > C$ with $C>0$ in \eqref{eq:A33}, together with \eqref{TcB_Upper_Fine_2}, yields a lower bound for the right side of \eqref{eq:A33}. This proves that $\Psi =0$. By \eqref{Second_Decomposition_alpha_equation} and \eqref{Second_Decomposition_Psi_xi_estimate}, this implies that $\alpha = 0$, i.e., $\Gamma$ is a diagonal state. Therefore, $\Gamma_0$ is the unique minimizer of $\FBCS$ in the temperature range \eqref{TcB_Upper_Fine_1} provided $D_0$ is chosen as above. This proves Theorem \ref{Main_Result_Tc}.























==> 6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc/6.4_Integral_representation_and_bound_rest_terms.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Proof of Lemma~\ref{Lower_Bound_B_remainings}}
\label{sec:A1}

In this section we prove Lemma~\ref{Lower_Bound_B_remainings}.
%\begin{lem}
%\label{Lower_Bound_B_remainings}
%We have the following estimates on the remainder terms of \eqref{LBpartB_3}:
%\begin{enumerate}[(a)]
%\item $|\langle \eta_\perp, [K_{\Tc,B}^r - K_{\Tc}^r]\sigma_0\rangle| \leq C B^3 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2$,
%
%\item $|\langle \eta_\perp, (U - 1) K_{\Tc,B}^r  \sigma_0\rangle| \leq C \varepsilon^{\nicefrac 12} B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2$,
%
%\item $|\langle \eta_\perp, UK_{\Tc,B}^r (U^* - 1)\sigma_0\rangle| \leq C \varepsilon^{\nicefrac 12} B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2$.
%\end{enumerate}
%\end{lem}
Our proof of part (a) uses a Cauchy integral representation for the operator $K_{\Tc,B}- (\pi^2 -\mu)$, which is provided in Lemma~\ref{KT_integral_rep} below. Let us start by defining the contour for the Cauchy integral.

\begin{defn}[Speaker path]
\label{speaker path}
Let $R>0$, assume that $\mu \leq 1$ and define the following complex paths 
\begin{align*}
\begin{split}
u_1(t) &:= \frac{\pi\i}{2\betac} + (1 + \i)t\\
%
u_2(t) &:= \frac{\pi\i}{2\betac} - (\mu + 1)t\\
%
u_3(t) &:= -\frac{\pi\i}{2\betac}t - (\mu + 1)\\
%
u_4(t) &:= -\frac{\pi\i}{2\betac} - (\mu + 1)(1-t) \\
%
u_5(t) &:= -\frac{\pi\i }{2\betac} + (1 - \i)t
\end{split}
&
\begin{split}
\phantom{ \frac \i\betac }t&\in [0,R], \\
%
\phantom{ \frac \i\betac }t &\in [0,1], \\
%
\phantom{ \frac \i\betac }t&\in [-1,1],\\
%
\phantom{ \frac \i\betac }t &\in [0,1],\\
%
\phantom{ \frac \i \betac }t&\in [0,R].
\end{split}
%
& \begin{split} 
\text{\includegraphics[width=6cm]{../BCS-Theory_General_Field/Speaker_path.pdf}}
\end{split} 
\end{align*}
The speaker path is defined as the union of paths $u_i$, $i=1, \ldots, 5$, with $u_1$ taken in reverse direction, i.e.,
\begin{align*}
\speaker_R := \mathop{\dot -}u_1 \mathop{\dot +} u_2 \mathop{\dot +} u_3 \mathop{\dot +} u_4 \mathop{\dot +} u_5.
\end{align*}
If $\mu > 1$ we choose the same path as in the case $\mu = 1$.
\end{defn} 
This path has the property that certain norms of the resolvent kernel of $\pi^2$ are uniformly bounded for $z \in \speaker_R$ and $R > 0$. More precisely, Lemma~\ref{GAz-GtildeAz_decay} implies
\begin{align}
\sup_{0\leq B\leq B_0} \sup_{R>0} \sup_{w\in \speaker_R} \bigl[ \left\Vert \, |\cdot |^a g_B^w\right\Vert_1 + \left \Vert \, |\cdot|^a \nabla g_B^w\right\Vert_1 \bigr] < \infty. \label{g0_decay_along_speaker}
\end{align}
We could also choose a path parallel to the real axis in Lemma~\ref{KT_integral_rep} below. In this case the above norms would depend on $R$. Although our analysis also works in this case, we decided to use the path $\speaker_R$ because of the more elegant bound in \eqref{g0_decay_along_speaker}. 
%This is obtained by combining the strategy of proof of Lemmas \ref{g0_decay} and \ref{gB-g_decay} with the estimate $(\Re \sqrt{-z})^2 \geq |\Re z|$, which holds as long as $\Re z \leq 0$. For $B_0 > 0$ sufficiently small and any $a\geq 0$, it is thus easy to show that for all $0 \leq B \leq B_0$, we have
With the above definition at hand, we are prepared to state the following lemma.

%We remark that it is not necessary for the following lemma to follow the paths $u_1$ and $u_5$. On the level of operators alone, as it is in Lemma \ref{KT_integral_rep}, we could indeed follow paths parallel to the real line. However, since we want to argue with kernels, we want to use uniform bounds on the resolvent kernel along the used path, see Lemma \ref{Gz_decay_along_speaker}. For the proof of this result, we utilize Lemma \ref{gz_decay}, whose bounds deteriorate along constant distance to the real line. This is the reason why we need to increase this distance linearly.

%For a well-defined contour integral, it would be sufficient to define the path parallel to the real axis, since the resolvent of the Laplacian is uniformly bounded as an operator and the function we are integrating is decaying sufficiently fast to make the integral convergent, see Lemma \ref{KT_integral_rep}. This is not true for the resolvent kernel. 
%However, with the contour defined above, we do have a uniform bound of the resolvent kernel along the contour. 

%We could give up uniformity (in $w$) in this bound and profit from an easier path, which could then be laid parallel to the real axis. The convergence of the contour integral in the following lemma would still be fine, since the underlying function is decaying exponentially fast as the real part of $w$ grows along the positive real line. However, with the method used to prove Lemma \ref{g0_decay}, we found it convenient to work with the speaker shaped path.

%\begin{lem}
%\label{g0_decay_along_speaker}
%For $a\geq 0$, we have
%
%%Here, $C_{\mu, T} = 2\tan(\frac 12 \arctan(\frac{\pi T}{2\mu_+}))^{-1}$. Likewise, for $a> -1$, we have
%%\begin{align*}
%%\sup_{w\in \speaker_{T,\mu}} \left\Vert \, |\cdot |^a \nabla g_0^w\right\Vert_{L^1(\Rbb^3)} < \infty.
%%\end{align*}
%\end{lem}

%\begin{proof}
%We apply Lemma \ref{gz_decay} by defining $\theta \in (0, \frac \pi 4]$ as
%\begin{align*}
%\theta &:= \frac 12 \arctan\bigl( \frac{\pi \Tc}{2\mu_+}\bigr).
%\end{align*}
%A similar proof to that of Lemma \ref{g0_decay} shows that the traces of $u_2, u_3$ and $u_4$ from Definition \ref{speaker path} belong to $S_\theta$. Concerning the path $u_1$, we remark that it has an angle of $\frac \pi 4$ from the starting point $t=0$, while the sector has an angle of at most $\frac \pi 4$. Hence, they do not intersect. Likewise for $u_5$. Thus, the speaker path lies in $S_\theta$.
%
%With the exception of $u_3$, we have $|\Im w| \geq \frac{\pi}{2\beta_c}$. By Lemma \ref{gz_decay}, for any $w\in \speaker_R \setminus \{u_3\}$, we thus have
%\begin{align*}
%\Vert \, |\cdot|^a g_0^w\Vert_1 \leq \Gamma(a+2) \;  C_\theta^{1+\frac a2} \;  \bigl(\frac{\pi}{2\beta_c}\bigr)^{-1-\frac a2}.
%\end{align*}
%
%For the path $u_3$, we provide the following addendum to the proof of Lemma \ref{gz_decay}. Since , we infer $(\Re \sqrt{-(w+\mu)})^2 \geq |\Re (w+\mu)|$ as long as $\Re w < -\mu$. Along $u_3$, we have $\Re w+\mu = -1$. Applying this to \eqref{Resolvent_kernel_integration} for $w\in u_3$, we get $\Vert \, |\cdot|^a g_0^w\Vert_1 \leq \Gamma(a+2)$. This proves claimed estimate on the first term of \eqref{g0_decay_along_speaker_2}.
%
%For the second term of \eqref{g0_decay_along_speaker_2}, employ  $|\sqrt{-(w+\mu)}| \leq |\Re w+\mu|^{\nicefrac 12} + |\Im w|^{\nicefrac 12}$. Combining this with \eqref{g0_decay_2} and \eqref{Resolvent_kernel_integration}, we get
%\begin{align}
%\Vert \, |\cdot|^a \nabla g_0^w\Vert_1 \leq \frac{|\Re w+\mu|^{\nicefrac 12} + |\Im w|^{\nicefrac 12}}{|\Re \sqrt{-(w+\mu)}|^{2+a}} \Gamma(a+2) + \frac{\Gamma(a+1)}{|\Re \sqrt{-(w+\mu)}|^{1+a}}. \label{g0_decay_along_speaker_3}
%\end{align}
%Along $u_3$, we apply the estimate $|\Re \sqrt{-(w +\mu)}| \geq C_\theta^{-\nicefrac 12} |\Im w|^{\nicefrac 12}$ as in \eqref{g0_decay_3} once to accomodate for the factor $|\Im w|$. For the remaining powers, we apply the lower bound $|\Re \sqrt{-(w+\mu)}|^2 \geq |\Re w+\mu|$ again, since $\Re w+\mu < 0$ here. This implies
%\begin{align*}
%\Vert \, |\cdot|^a \nabla g_0^w\Vert_1 \leq \; \bigl( \Gamma(a+2) + \Gamma(a+1) + C_\theta^{\nicefrac 12}\bigr) \; |\Re w + \mu|^{-\frac 12 - \frac a2}.
%\end{align*}
%Since $\Re w + \mu = -1$ along $u_3$, we conclude the uniform bound. 
%
%On the remainder of the speaker path, we have $|\Im w|\geq \frac{\pi}{2\beta_c}$. Therefore, using \eqref{g0_decay_3} and \eqref{g0_decay_along_speaker_3},
%\begin{align}
%\Vert \, |\cdot|^a \nabla g_0^w\Vert_1 \leq \Bigl[ \Gamma(a+2) C_\theta^{1 + \frac a2} \frac{|\Re w+\mu|^{\nicefrac 12} + |\Im w|^{\nicefrac 12}}{|\Im w|^{\nicefrac 12}} + \Gamma(a+1) C_\theta^{\frac 12+\frac a2}\Bigr] |\Im w|^{-\frac 12 - \frac a2}. \label{g0_decay_along_speaker_1}
%\end{align}
%Inserting the explicit form of $w+\mu$ in the segments of $\speaker_R$ into \eqref{g0_decay_along_speaker_1}, we see that the term in square brackets is uniformly bounded.
%
%
%
%
%
%\begin{align}
%\Vert \, |\cdot|^a \nabla g_0^z\Vert_1 \leq \Bigl[ \Gamma(a+2) C_{\mu, T}^{1 + \frac a2} \frac{|\Re z+\mu|^{\nicefrac 12} + |\Im z|^{\nicefrac 12}}{|\Im z|^{\nicefrac 12}} + \Gamma(a+1) C_{\mu, T}^{\frac 12+\frac a2}\Bigr] |\Im z|^{-\frac 12 - \frac a2}
%%
%%
%%
%%
%%\frac{|\Re z+\mu|^{\nicefrac 12} + |\Im z|^{\nicefrac 12}}{|\Re \sqrt{-(z+\mu)}|^{2+a}} \Gamma(a+2) + \frac{\Gamma(a+1)}{|\Re \sqrt{-(z+\mu)}|^{1+a}}. 
%\label{g0_decay_along_speaker_1}
%\end{align}
%We applied the estimate $|\Re \sqrt{-(z +\mu)}| \geq C_{\mu, T}^{-\nicefrac 12} |\Im z|^{\nicefrac 12}$ as in \eqref{g0_decay_3}. 
%%For the remaining powers, we apply $|\Re \sqrt{-(z+\mu)}|^2 \geq |\Re z+\mu|$. This implies
%%\begin{align*}
%%\Vert \, |\cdot|^a g_0^z\Vert_1 \leq \Gamma(a+2) \; (2+ C_{\mu, T}^{\nicefrac 12}) \; |\Re z + \mu|^{-\frac 12 - \frac a2}.
%%\end{align*}
%%Since $\Re z + \mu = -1$ along $u_3$, we conclude the uniform bound. 
%Inserting the explicit form of $z+\mu$ in the segments of $\speaker_{T, \mu}$ in to \eqref{g0_decay_along_speaker_1}, we see that the term in square brackets is uniformly bounded.
%\end{proof}

%\notiz{We could give up uniformity of the bound \eqref{g0_decay_along_speaker} for simplifying the speaker path to a parallel-to-the-real-axis path. It does not disturb the convergence of the integral but makes the derivation of \eqref{g0_decay_along_speaker} more tedious, since we need to analyse the rate of deterioration of $\Vert g_0^w\Vert_1$. It will be linear in $\Re z$ for $\Re z \gg 1$. Shall we do that? Does not simplify much more than that, I think.}

\begin{lem}
\label{KT_integral_rep}
Let $H\colon \Dcal(H)\ra \Hcal$ be a self-adjoint operator on a separable Hilbert space~$\Hcal$ with $H\geq -\mu$. Then, we have
\begin{align}
\frac{H}{\tanh(\frac{\betac}{2} H)} = H + \lim_{R\to\infty} \int_{\speaker_R} \frac{\dd z}{2\pi\i} \Bigl( \frac{z}{\tanh(\frac{\betac}{2} z)} - z \Bigr) \frac{1}{z - H}, \label{KT_integral_rep_eq}
\end{align}
with the speaker path $\speaker_R$ in Definition~\ref{speaker path}. The above integral including the limit is understood as an improper Riemann integral with respect to the uniform operator topology.  
\end{lem}

\begin{proof}
We have that the function $f(z) = \frac{z}{\tanh(\frac{\betac }{2}z)} - z = \frac{2z}{\e^{\betac z} - 1}$ is analytic in the open domain $\Cbb \setminus 2\pi T \i \Zbb_{\neq 0}$. The construction of the Riemann integral over the path $\speaker_R$ with respect to the uniform operator topology is standard. The fact that the limit $R \to \infty$ exists in the same topology follows from the exponential decay of the function $f(z)$ along the speaker path. To check the equality in \eqref{KT_integral_rep_eq}, we evaluate both sides in the inner product with two vectors in $\ran \Idbb_{(-\infty, K]}(H)$ for $K > 0$ and use the functional calculus, the Cauchy integral formula and the fact that $\bigcup_{K>0} \ran \Idbb_{(-\infty, K]}(H)$ is a dense subset of $\Hcal$. This proves the claim.
\end{proof}


 

%and on the interval $[-\mu, \infty)$ we have $\Vert f\Vert_\infty = \frac{2\mu}{1 - \e^{-\betac \mu}}$. Therefore, $f(H)$ is a bounded operator.

%A straightforward computation shows that the limit on the right side of \eqref{KT_integral_rep_eq} exists in operator norm and defines a bounded operator that we denote by $g(H)$.
%We prove that the limit 
%\begin{align*}
%g(H) := \lim_{R\to\infty} \int_{\speaker_R} \frac{\dd z}{2\pi\i} \; f(z) \, \frac{1}{z - H}
%\end{align*}
%exists and defines a bounded operator on $\Hcal$. To do this, we investigate the tails of the paths $u_1$ and $u_5$. For example, we have to investigate the operator norm of
%\begin{align*}
%\int_R^\infty \frac{\dd t}{2\pi\i} \frac{2u_1(t)}{\e^{\betac u_1(t)} - 1} \frac{1}{u_1(t) - H} \;  u_1'(t).
%\end{align*}
%Note the following simple estimates for $t$ large enough
%\begin{align*}
%|u_1(t)| &\leq \frac{\pi}{2\betac} + \sqrt{2} t \leq Ct, & |u_1'(t)| &= \sqrt{2}, & \Re u_1(t) &= t,
%\end{align*}
%as well as
%\begin{align*}
%\Vert (u_1(t) - H)^{-1}\Vert_\infty &\leq \frac{1}{\Im u_1(t)} = \frac{1}{\frac{\pi}{2\betac} + t} \leq \frac 1t.
%\end{align*}
%This implies that
%\begin{align*}
%\Bigl\Vert \int_R^\infty \frac{\dd t}{2\pi\i} \frac{2u_1(t)}{\e^{\betac u_1(t)} - 1} \frac{1}{u_1(t) - H} \;  u_1'(t)\Bigr\Vert_\infty &\leq C \int_R^\infty \frac{1}{\e^{\betac t} - 1} \leq C \e^{-\betac R}.
%\end{align*}
%The contribution of $u_5$ is estimated in a similar fashion. This proves operator norm convergence of the limit and that $g(H)$ is bounded.

%Let $K \geq 0$ and choose $\eta\in \ran(\Idbb_{(-\infty, K-1]}(H))$. Take $R\geq K$ and close the speaker path by the contour $u_R(t) := R + (R+ \frac{\pi}{2\betac}) \i t$ where $t\in [-1,1]$. The Cauchy integral formula shows 
%\begin{align*}
%\langle \varphi, f(H) \eta\rangle = \int_{\speaker_R \dot + u_R} \frac{\dd z}{2\pi\i} \; f(z) \, \langle \varphi, (z - H)^{-1} \eta\rangle.
%\end{align*}
%for $\varphi\in \Hcal$. It remains to show that the integral over $u_R$ vanishes as $R \to \infty$. We use
%\begin{align*}
%\Bigl|\int_{u_R} \frac{\dd z}{2\pi\i} \; f(z) \langle \varphi, (z - H)^{-1}\eta\rangle\Bigr| &\leq \int_{-1}^1 \frac{\dt}{\pi} \frac{|u_R(t)|}{|\e^{\betac u_R(t)}| - 1} \;  |\langle \varphi, (u_R(t) - H)^{-1} \eta\rangle|\;  |u_R'(t)|.
%\end{align*}
%Since $\Re u_R(t) = R$, we have
%$|u_R(t) - (K-1)| \geq 1$ to see that $\sup_{t\in [-1,1]}\Vert (u_R(t) - H)^{-1}\Idbb_{(-\infty, K-1]}(H)\Vert_\infty \leq 1$. The claim follows from the decay of $f$ on the path $u_R(t)$. 
% Hence, we obtain
%\begin{align*}
%\sup_{\Vert \varphi\Vert = 1} \Bigl|\int_{u_R} \frac{\dd z}{2\pi\i} \; f_{\Tc}(z) \langle \varphi, (z - H)^{-1}\eta\rangle\Bigr| &\leq C \;  \frac{R^2}{\e^{\betac R} - 1} \;  \Vert\eta\Vert \xra{R\to\infty} 0.
%\end{align*}
%We conclude that the second term on the right side of \eqref{KT_integral_rep_eq} equals $f(H)$. This proves the claim. %Since both operators are bounded, this extends to all $\eta\in \Hcal$ by density. %Since $H$ and $\frac{H}{\tanh(\frac{\betac}{2} H)}$ have the same domain $\Dcal(H)$, the claim holds for all $\eta\in \Dcal(H)$.


Henceforth, we use the symbol $\int_{\speaker}$ to denote the integral on the right side of \eqref{KT_integral_rep_eq} including the limit and we denote $\speaker = \bigcup_{R > 0} \speaker_R$.

\begin{proof}[Proof of Lemma \ref{Lower_Bound_B_remainings}]
%Throughout we use the estimates of Theorems \ref{Structure_of_alphaDelta} and \ref{Structure_of_almost_minimizers}, as well as $B \leq \varepsilon \leq 1$.
We apply Cauchy-Schwarz to estimate
\begin{align}
|\langle \eta_\perp, (K_{\Tc,B}^r - K_{\Tc}^r)\sigma_0\rangle| \leq \Vert \eta_\perp\Vert_2 \, \Vert (K_{\Tc,B}^r- K_{\Tc}^r)\sigma_0\Vert_2
\label{eq:A34}
\end{align}
and claim that 
\begin{align}
\Vert [K_{{\Tc},B}^r - K_{\Tc}^r]\sigma_0\Vert_2 \leq C \varepsilon^{-\nicefrac 12} B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)} \label{Lower_Bound_B_remainings_3}
\end{align}
holds. To see this, we apply Lemma~\ref{KT_integral_rep} and write
\begin{align}
K_{{\Tc},B}^r - K_{\Tc}^r = \pi_r^2 - p_r^2 + \int_\speaker \frac{\dd w}{2\pi\i} \; f(w) \;  \frac{1}{w + \mu - \pi_r^2} [\pi_r^2 - p_r^2] \frac{1}{w + \mu - p_r^2}, \label{Lower-bound-final_2}
\end{align}
where $\pi_r^2 - p_r^2 = \i \, \Bbold\wedge r\;  p_r + \frac 14 |\Bbold\wedge r|^2$. Using \eqref{Psi>_bound} and \eqref{Decay_of_alphastar}, we estimate the first term on the right side of \eqref{Lower-bound-final_2} by
\begin{align}
\Vert [\pi_r^2 - p_r^2]\sigma_0\Vert_2 &\leq B \, \Vert \, |\cdot|\nabla \alpha_*\Vert_2 \Vert \Psi_>\Vert_2 + B^2 \Vert \,|\cdot|^2\alpha_*\Vert_2 \Vert \Psi_>\Vert_2 \notag\\
%
&\leq C\varepsilon^{-\nicefrac 12} B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}. \label{Lower_Bound_B_remainings_1}
\end{align}
To estimate the second term in \eqref{Lower-bound-final_2}, we use Hölder's inequality in \eqref{Schatten-Hoelder} and find
\begin{align*}
\Bigl\Vert \int_\speaker \frac{\dd w}{2\pi\i} \, f(w)\;  \frac{1}{w + \mu - \pi_r^2} [\pi_r^2 - p_r^2]\frac{1}{w+\mu - p_r^2}\sigma_0\Bigr\Vert_2 &\\
%
&\hspace{-180pt}\leq \int_\speaker \frac{\dd |w|}{2\pi}\,  |f(w)| \, \Bigl\Vert \frac{1}{w + \mu- \pi_r^2} \Bigr\Vert_\infty \Bigl\Vert [\pi_r^2 - p_r^2]\frac{1}{w + \mu - p_r^2}\sigma_0\Bigr\Vert_2,
\end{align*}
where $\dd |w| = \dd t \; |w'(t)|$. Eq.~\eqref{g0_decay_along_speaker} implies that the operator norm of the magnetic resolvent is uniformly bounded for $w \in \speaker$. Since the function $f$ is exponentially decaying along the speaker path it suffices to prove a bound on the last factor that is uniform for $w \in \speaker$. We have
\begin{align*}
[\pi_r^2 - p_r^2] \frac{1}{w + \mu - p_r^2} \sigma_0(X,r) &= \int_{\Rbb^3} \dd s \; [\pi_r^2 - p_r^2] g_0^w(r - s) \alpha_*(s) \Psi_>(X),
\end{align*}
which implies
\begin{align}
\Bigl\Vert [\pi_r^2 - p_r^2] \frac{1}{w + \mu - p_r^2}\sigma_0\Bigr\Vert_2^2 &
%\leq\\
%%
%&\hspace{-100pt}\leq \int_{\Rbb^3} \dd r \int_{\Rbb^3} \dd s \int_{\Rbb^3} \dd s' \; |[\pi_r^2 - p_r^2]G^w(r - s) \alpha_*(s)|\cdot |[\pi_r^2 - p_r^2]G^w(r - s') \alpha_*(s')|\\
%%
%& \times \fint_{Q_B} \dd X \; \bigl| \cos\bigl(\frac{s}{2}\Pi_X\bigr) \Psi_>(X)\bigr| \;  \bigl|\cos\bigl( \frac{s'}{2}\Pi_X\bigr) \Psi_>(X)\bigr|\\
%
\leq \Vert \Psi_>\Vert_2^2 \int_{\Rbb^3} \dd r \, \Bigl| \int_{\Rbb^3} \dd s \; |[\pi_r^2 - p_r^2] g_0^w(r - s) \alpha_*(s)|\Bigr|^2. \label{Lower_Bound_B_remainings_2}
\end{align}
Moreover,
%note that
%\begin{align*}
%|[\pi_r^2 - p_r^2] G^w(r - s) \alpha_*(s)| &\leq B |r - s||G^w(r - s)| |\alpha_*(s)| + B |G^w(r - s)| \;  |s||\alpha_*(s)| \\
%%
%&\hspace{0pt} + B^2 |r - s|^2 |G^w(r - s)| |\alpha_*(s)| + B^2 |G^w(r - s)| |s|^2 |\alpha_*(s)|.
%\end{align*}
%This implies
\begin{align*}
\int_{\Rbb^3} \dd r \; \Bigl| \int_{\Rbb^3} \dd s \; |[\pi_r^2 - p_r^2] g_0^w(r - s) \alpha_*(s)|\Bigr|^2 & \\
%
&\hspace{-195pt} \leq CB^2 \bigl( \Vert \, |\cdot| \nabla g_0^w\Vert_1^2 \; \Vert \alpha_*\Vert_2^2 + \Vert \nabla g_0^w\Vert_1^2 \; \Vert \, |\cdot|\alpha_*\Vert_2^2 + \Vert \,  |\cdot|^2 g_0^w\Vert_1^2 \;  \Vert\alpha_*\Vert_2^2 + \Vert g_0^w\Vert_1^2 \;  \Vert \, |\cdot|^2\alpha_*\Vert_2^2\bigr).
\end{align*}
The right side is uniformly bounded for $w \in \speaker$ by \eqref{g0_decay_along_speaker} and \eqref{Decay_of_alphastar}. In combination with \eqref{Psi>_bound} and \eqref{Lower_Bound_B_remainings_2}, this implies
\begin{align*}
\Bigl\Vert [\pi_r^2 -p_r^2]\frac{1}{w + \mu - p_r^2} \sigma_0\Bigr\Vert_2^2 & \leq CB^2 \;  \Vert\Psi_>\Vert_2^2\leq C \varepsilon^{-1} B^4 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2.
\end{align*}
Using this and \eqref{Lower_Bound_B_remainings_1}, we read off \eqref{Lower_Bound_B_remainings_3}. Finally, we apply Proposition~\ref{Structure_of_alphaDelta} to estimate $\Vert \eta_\perp\Vert_2$ in \eqref{eq:A34}, which proves part (a).

%\item  $K_{T,B}^r - K_{\Tc,B}^r$ is a bounded operator of order $B$, as argued in \eqref{KTc_bounded_derivative}. Hence
%\begin{align*}
%|\langle \eta_\perp, [K_{T,B}^r - K_{\Tc,B}^r]\sigma_0\rangle| &\leq CB \;  \Vert \eta_\perp\Vert_2 \;  \Vert \sigma_0\Vert_2 \leq CB \varepsilon^{\nicefrac 12} B^{\nicefrac 14} \;  \varepsilon^{-\nicefrac 12} B^{\nicefrac 14} \leq CB^{\nicefrac 32}.
%\end{align*}

To prove part (b), we start by noting that
\begin{align*}
|\langle \eta_\perp, (U-1) K_{\Tc,B}^r\sigma_0 \rangle| &\leq \Vert \,  |r| \eta_\perp\Vert_2 \;  \Vert\, |r|^{-1} (U - 1) K_{\Tc,B}^r \, \sigma_0 \Vert_2. %\label{Lower_Bound_B_remainings_5}
\end{align*}
A bound for the left factor on the right side is provided by Proposition~\ref{Structure_of_alphaDelta}. To estimate the right factor, we use \eqref{Psi>_bound}, \eqref{Decay_of_alphastar} and the operator inequality in \eqref{ZPiX_inequality}, which implies $|U- 1|^2 \leq 3 r^2 \Pi_X^2$, and find
\begin{align*}
\Vert\, |r|^{-1} (U - 1) K_{\Tc,B}^r \, \sigma_0 \Vert_2 &\leq C \Vert K_{\Tc,B}^r \alpha_*\Vert_2 \; \Vert \Pi\Psi_>\Vert_2 \leq CB \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}.
\end{align*}
This proves part (b).
%Using $K_{\Tc,B}^r \leq C(1+\pi_r^2)$, we obtain
%\begin{align*}
%\bigl\Vert \sqrt{K_{\Tc,B}^r} \, \sigma_0\bigr\Vert^2 &= \langle \sigma_0, K_{\Tc,B}\sigma_0\rangle \leq C ( \Vert \sigma_0\Vert_2^2 + \Vert \pi_r\sigma_0\Vert_2^2) \leq C \varepsilon^{-1} B^ {\nicefrac 12}.
%\end{align*}
%\notiz{Indizes der Normen}Turning to the left factor in \eqref{Lower_Bound_B_remainings_5}, we have 
%\begin{align}
%\Vert \sqrt{K_{\Tc,B}} (U-1) \eta_\perp\Vert^2 &\leq \Vert (U-1) \eta_\perp\Vert^2 + \Vert \pi_r (U-1) \eta_\perp\Vert^2. \label{Lower_Bound_B_remainings_4}
%\end{align}
%Using Theorem \ref{Structure_of_alphaDelta} and \eqref{Psi_Higher_Derivatives} for $k =3$, the left term is bounded by
%\begin{align*}
%\Vert (U-1) \eta_\perp\Vert^2 &\leq \Vert \, |r\Pi_X| \eta_\perp\Vert^2 \leq C \, B^{\nicefrac 52} \;  (\varepsilon B^{-1})^2 \leq C \varepsilon^2 B^{\nicefrac 12}.
%\end{align*}
%By the intertwining relations in Lemma \ref{CommutationI}, we have
%\begin{align*}
%\pi_r (U-1) = (U-1) \tilde \pi_r - \frac 12 U \Pi_X - \frac 14 \Bbold \wedge r. %\label{Lower-bound-final_1}.
%\end{align*}
%Using this, the right term of \eqref{Lower_Bound_B_remainings_4} is bounded by
%\begin{align*}
%\Vert \pi_r (U-1) \eta_\perp \Vert^2 &\leq C \bigl( \Vert |r\Pi_X|\tilde \pi_r\eta_\perp\Vert^2 + \Vert \Pi_X\eta\Vert^2 + B^2 \Vert |r|\eta_\perp\Vert^2\bigr) \leq C \varepsilon^2 B^{\nicefrac 12}.
%\end{align*}

For part (c), we estimate
\begin{align}
|\langle \eta_\perp, UK_{\Tc,B}^r (U^* - 1) \sigma_0\rangle|  &\leq \bigl\Vert \sqrt{K_{\Tc,B}^r} \, U^* \eta_\perp \bigr\Vert_2 \;  \bigl\Vert \sqrt{K_{\Tc,B}^r}\, (U^* - 1)\sigma_0\bigr\Vert_2
\label{eq:A35}
\end{align}
and note that $K_{\Tc,B}^r \leq C(1+ \pi_r^2)$ implies
\begin{align}
\bigl\Vert \sqrt{K_{\Tc,B}^r} (U^* - 1)\sigma_0\bigr\Vert_2^2 &= \langle \sigma_0, (U - 1) K_{\Tc,B}^r (U^* - 1)\sigma_0\rangle \notag\\
%
&\leq C \Vert (U^* - 1)\sigma_0\Vert_2^2 + C\Vert \pi_r (U^* - 1)\sigma_0\Vert_2^2.\label{Lower-bound-final_3}
\end{align}
Using the bound for $|U-1|^2$ in part (b), \eqref{Psi>_bound} and \eqref{Decay_of_alphastar}, we see that the first term is bounded by $C\Vert |r|\alpha_* \Pi_X\Psi_>\Vert^2 \leq CB^2$. Lemma~\ref{CommutationI} allows us to write
\begin{align*}
\pi_r (U^* - 1) &= (U^* - 1) \tilde \pi_r + \frac 12 U^*\Pi_X - \frac 14 \Bbold \wedge r.
\end{align*}
Accordingly, we have
\begin{align*}
\Vert \pi_r (U^* - 1)\sigma_0\Vert_2^2 &\\
%
&\hspace{-50pt}\leq C\bigl( \Vert \, |r| p_r\alpha_*\Pi_X\Psi_>\Vert_2^2 + B \, \Vert \, |r|^2\alpha_* \Pi_X \Psi_> \Vert_2^2 + \Vert \alpha_*\Pi_X\Psi_>\Vert_2^2 + B \Vert \, |r|\alpha_* \Psi_>\Vert_2^2\bigr)\\
%
&\hspace{-50pt}\leq C \bigl( B^2 + \varepsilon^{-1} B^3 \bigr) \leq CB^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2.
\end{align*}
We conclude that the right side of \eqref{Lower-bound-final_3} is bounded by $CB^2 \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2$. 

With $K_T(p) \leq C (1+p^2)$ we see that the first factor on the right side of \eqref{eq:A35} is bounded by
\begin{align*}
\bigl\Vert \sqrt{K_{\Tc,B}^r} \, U^* \eta_\perp\bigr\Vert_2^2 &= \langle \eta_\perp , U K_{\Tc,B}^r U^* \eta_\perp\rangle \leq C \Vert \eta_\perp\Vert_2^2 + C\Vert \pi_rU^*\eta_\perp\Vert_2^2.
\end{align*}
From Lemma~\ref{CommutationI} we know that $\pi_r U^* = U^* [\tilde\pi_r + \frac 12 \Pi_X]$, and hence
\begin{align*}
\bigl\Vert \sqrt{K_{\Tc,B}^r} \, U^* \eta_\perp\bigr\Vert_2^2 &\leq C \bigl( \Vert \eta_\perp\Vert_2^2 + \Vert \tilde \pi_r\eta_\perp\Vert_2^2 + \Vert \Pi_X\eta_\perp\Vert_2^2\bigr) \leq C \varepsilon B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2. 
\end{align*}
This proves part (c) and ends the proof.
\end{proof}
